Toward Long-Term and Archivable Reproducibility

Analysis pipelines commonly use high-level technologies that are popular when created, but are unlikely to be readable, executable, or sustainable in the long term. A set of criteria is introduced to address this problem: Completeness (no execution requirement beyond a minimal Unix-like operating system, no administrator privileges, no network connection, and storage primarily in plain text); modular design; minimal complexity; scalability; verifiable inputs and outputs; version control; linking analysis with narrative; and free and open source software. As a proof of concept, we introduce "Maneage" (Managing data lineage), enabling cheap archiving, provenance extraction, and peer verification that has been tested in several research publications. We show that longevity is a realistic requirement that does not sacrifice immediate or short-term reproducibility. The caveats (with proposed solutions) are then discussed and we conclude with the benefits for the various stakeholders. This article is itself a Maneage'd project (project commit 54e4eb2).

==> project <==
#!/bin/sh
#
# High-level script to manage the project.
# Run './project --help' for a description of how to use it.
#
# Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
# Copyright (C) 2021-2022 Raul Infante-Sainz <infantesainz@gmail.com>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.


# Basic settings
# --------------
# Stop the script if there are any errors.
set -e





# Default option values
jobs=0     # 0 is for the default for the 'configure.sh' script.
group=
debug=
host_cc=0
operation=
build_dir=
input_dir=
check_config=
make_targets=
software_dir=
clean_texdir=0
prepare_redo=0
highlightnew=0
all_highlevel=0
existing_conf=0
highlightnotes=0
separatesupplement=0
scriptname="./project"





# Parse the options
# -----------------
#
# Separate command-line arguments from options. Then put the option value
# into the respective variable.
#
# Each option has two lines because we want to process both these formats:
# '--name=value' and '--name value'. The former (with '=') is a single
# command-line argument, so we just need to shift the counter by one. The
# latter (without '=') is two arguments, so we'll need two shifts.
#
# Note on the case strings: for every option, we need three lines: one when
# the option name and value are separate. Another when there is an equal
# between them, and finally one where the value is immediately after the
# short-format. This exact order is important. Otherwise, there will be a
# conflict between them.

print_help() {
    # Print the output.
    cat <<EOF
Usage: $scriptname configure [OPTIONS]
       $scriptname shell     [OPTIONS]
       $scriptname make      [OPTIONS]

Top-level script to manage the reproducible project. The high-level
operation is defined by the (mandatory) second argument:

  configure    - Configure project for this machine (e.g., build software).
  make         - Run the project (do analysis and build outputs).
  shell        - Execute the project's shell for interactive testing.

RECOMMENDATION: If this is the first time you are configuring this
template, please don't use the options and let the script explain each
parameter in full detail by simply running './project configure'.

Project 'make' special features.
  ./project make           Build the project on one thread
  ./project make -jN       Built the project in parallel on N threads.
  ./project make clean     Clean all files generated by 'make' (not software).
  ./project make texclean  Clean all files built by (La)TeX.
  ./project make distclean Clean everything (including compiled software).
  ./project make dist      Produce a LaTeX-ready-to-build distribution tarball
                           ('tar.gz') of the project. This is ready to be
                           uploaded to servers like 'arXiv.org'.
  ./project make dist-lzip Similar to 'dist', but compress to '.tar.lz'.
  ./project make dist-zip  Similar to 'dist', but compress to '.zip'.
  ./project make dist-software  Build a .tar.gz tarball containing all
                                software source tarballs necessary for the
                                project.

With the options below you can modify the default behavior.
Configure options:
  -b, --build-dir=STR      Top directory to build the project in.
  -e, --existing-conf      Use (possibly existing) local configuration.
      --host-cc            Use host system's C compiler, don't build GCC.
  -i, --input-dir=STR      Directory containing input datasets (optional).
  -s, --software-dir=STR   Directory containing necessary software tarballs.
      --check-config       During configuration, show what is being built.
      --clean-texdir       Remove possibly existing build-time subdirectories
                           under the project's 'tex/' directory (can happen
                           when source is from arXiv for example).
      --all-highlevel      Build all high-level software (for development).

Configure and Make options:
  -d, --debug[=FLAGS]      In configure: use -j1, no -k, and no Zenodo check.
                           In make: 'FLAGS' will be directly passed to 'make'.
  -g, --group=STR          Build and run with write permissions for a group.
  -j, --jobs=INT           Number of threads to build/run the software.
  -?, --help               Print this help list.

Make (analysis) options:
  -p, --prepare-redo       Re-do preparation (only done automatically once).

Make (final PDF) options:
      --refresh-bib        Force refresh the bibliography.
      --highlight-new      Highlight '\new' parts of text as green.
      --highlight-notes    Show '\tonote' regions as red text in PDF.
      --supplement         Build the appendices as a separate supplement PDF.

Mandatory or optional arguments to long options are also mandatory or optional
for any corresponding short options.

Maneage URL: https://maneage.org

Report bugs to mohammad@akhlaghi.org
EOF
}

on_off_option_error() {
    if [ "x$2" = x ]; then
        echo "$scriptname: '$1' doesn't take any values."
    else
        echo "$scriptname: '$1' (or '$2') doesn't take any values."
    fi
    exit 1
}

check_v() {
    if [ x"$2" = x ]; then
        echo "$scriptname: option '$1' requires an argument."
        echo "Try '$scriptname --help' for more information."
        exit 1;
    fi
}

func_operation_set() {
    if [ x$operation = x ]; then
        operation=$1
    else
        echo "Only one operation ('configure', 'make' or 'shell') may be given."
        exit 1
    fi
}

while [ $# -gt 0 ]
do
 case $1 in
  # Main operation.
  configure)    func_operation_set $1; shift;;
  make)         func_operation_set $1; shift;;
  shell)        func_operation_set $1; shift;;

  # Configure options:
  -b|--build-dir)        build_dir="$2";                                     check_v "$1" "$build_dir";    shift;shift;;
  -b=*|--build-dir=*)    build_dir="${1#*=}";                                check_v "$1" "$build_dir";    shift;;
  -b*)                   build_dir=$(echo    "$1" | sed -e's/-b//');         check_v "$1" "$build_dir";    shift;;
  -e|--existing-conf)    existing_conf=1;                                                                  shift;;
  -e*|--existing-conf=*) on_off_option_error --existing-conf -e;;
  --host-cc)             host_cc=1;                                                                        shift;;
  --host-cc=*)           on_off_option_error --host-cc;;
  -i|--input-dir)        input_dir="$2";                                     check_v "$1" "$input_dir";    shift;shift;;
  -i=*|--input-dir=*)    input_dir="${1#*=}";                                check_v "$1" "$input_dir";    shift;;
  -i*)                   input_dir=$(echo    "$1" | sed -e's/-i//');         check_v "$1" "$input_dir";    shift;;
  -s|--software-dir)     software_dir="$2";                                  check_v "$1" "$software_dir"; shift;shift;;
  -s=*|--software-dir=*) software_dir="${1#*=}";                             check_v "$1" "$software_dir"; shift;;
  -s*)                   software_dir=$(echo "$1" | sed -e's/-s//');         check_v "$1" "$software_dir"; shift;;
  --check-config)        check_config=1;                                                                   shift;;
  --check-config=*)      on_off_option_error --check-config;;
  --clean-texdir)        clean_texdir=1;                                                                   shift;;
  --clean-texdir=*)      on_off_option_error --clean-texdir;;
  --all-highlevel)       all_highlevel=1;                                                                  shift;;
  --all-highlevel=*)     on_off_option_error --all-highlevel;;

  # Configure and Make options:
  -g|--group)             group="$2";                            check_v group "$group";   shift;shift;;
  -g=*|--group=*)         group="${1#*=}";                       check_v group "$group";   shift;;
  -g*)                    group=$(echo   "$1" | sed -e's/-g//'); check_v group "$group";   shift;;
  -j|--jobs)              jobs="$2";                             check_v jobs  "$jobs";    shift;shift;;
  -j=*|--jobs=*)          jobs="${1#*=}";                        check_v jobs  "$jobs";    shift;;
  -j*)                    jobs=$(echo "$1" | sed -e's/-j//');    check_v jobs  "$jobs";    shift;;
  -'?'|--help)            print_help; exit 0;;
  -'?'*|--help=*)         on_off_option_error --help -?;;

  # Make options
  # ------------
  #
  # Note that Make's `debug' can take values, but when called without any
  # value, it is like giving it a value of `a'):
  --supplement)           separatesupplement=1;                                            shift;;
  --supplement=*)         on_off_option_error --supplement;;

  # Note that Make's 'debug' can take values, but when called without any
  # value, it is like giving it a value of 'a'):
  --refresh-bib)          [ -f tex/src/references.tex ] && touch tex/src/references.tex;   shift;;
  --highlight-new)        highlightnew=1;                                                  shift;;
  --highlight-new=*)      on_off_option_error --highlight-new;;
  --highlight-notes)      highlightnotes=1;                                                shift;;
  --highlight-notes=*)    on_off_option_error --highlight-notes;;
  -d|--debug)             if [ x$operation = x ]; then
                              echo "Please set the operation before calling '--debug'"; exit 1
                          elif [ x$operation = xconfigure ]; then debug=a;   shift;
                          elif [ x$operation = xmake ]; then
                              if [ x"$2" = x ]; then echo "In make-mode, '--debug' needs a value"; exit 1
                              else debug="$2"; check_v debug "$debug"; shift;shift; fi
                          else
                              echo "Operation '$operation' not recognized, please use 'configure' or 'make'"
                          fi;;
  -d=*|--debug=*)         debug="${1#*=}";                       check_v debug "$debug";   shift;;
  -d*)                    debug=$(echo "$1" | sed -e's/-d//');   check_v debug "$debug";   shift;;
  -p|--prepare-redo)      prepare_redo=1;                                                  shift;;
  -p=*|--prepare-redo=*)  on_off_option_error --prepare-redo;                              shift;;

  # Unrecognized option:
  -*) echo "$scriptname: unknown option '$1'"; exit 1;;

  # Not an option, an argument (so its a Make target).
  *) make_targets="$make_targets $1"; shift;;
 esac
done





# Check configuration status
# --------------------------
if ! [ x$check_config = x ]; then
    # Find the color option to pass to 'ls'. Note that '--color' (for GNU
    # Coreutils 'ls') should be checked first because it also has '-G', but
    # for something else.
    if   ls --color 2> /dev/null > /dev/null; then coloropt="--color=auto"
    elif ls -G      2> /dev/null > /dev/null; then coloropt="-G"
    else                               coloropt=""
    fi

    # Print a notice to let the user know what is happening.
    cat <<EOF

This is an infinite loop that will print what software are being built at
every moment. It is actually a listing ('ls' command) of the temporary
directory where software source code are unpacked while they are being
built. If the project isn't being configured, the output (every second)
will either be empty (only a date) or a with an error about a non-existant
directory. This feature is thus only useful when the project's software are
being built.

EOF

    # Run the infinite loop. To be able to find the last built programs, we
    # need to put all the Python programs and high-level program into one
    # directory.
    checkdir=.local/version-info/.for-check-config
    while true; do

        # Make sure the '.build' directory has already been created.
        echo;
        echo "========================"
        if [ -d .build ]; then
            echo "$(date)    [[press CTRL-C to stop]]";
            echo "--- Currently being built:"
            if [ -d .build/software/build-tmp ]; then
                ls $coloropt .build/software/build-tmp || junk=1;
            fi

            # Make the temporary directory, delete its contents, then put new
            # links of all built software.
            if ! [ -d $checkdir ]; then mkdir $checkdir; fi
            rm -f $checkdir/*

            # Check if any programs exist in the given directory yet.
            printresults=0
            check=$(ls .local/version-info/python/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/python/*  $checkdir/
            fi
            check=$(ls .local/version-info/proglib/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/proglib/* $checkdir/
            fi

            # If something was actually found, then print them.
            if [ $printresults = 1 ]; then
                echo "--- Last 5 packages that were built:"

                # Then sort all the links based on the most recent dates of the
                # files they link to (with '-L').
                ls -Llt $checkdir  \
                    | awk '/^-/ && c++<5 {printf "[at %s] %s\n", $(NF-1), $NF}'
            fi
        else
            cat <<EOF
The connection to the build directory (.build) is not yet created.

If you have just ran './project configure', it should be created and will
be used in a few seconds to report the build status of various software.
If not, please run './project configure' (in another terminal) and you will
see the results shortly afterwards.
EOF
        fi
        echo "========================"

        # Wait for the next round of checks.
        sleep 1
    done
    exit 0
fi





# Basic group settings
# --------------------
if ! [ x$group = x ]; then

    # Check if group is usable.
    if ! sg "$group" "echo Group \'$group\' exists"; then
        echo "$scriptname: '$group' is not a usable group name on this system.";
        echo "(TIP: you can use the 'groups' command to see your groups)"
        exit 1
    fi

    # Set the group option for running Make.
    gopt="maneage_group_name=$group"
fi





# Error when configuration isn't run
configuration_necessary() {
    cat <<EOF

The project is either (1) not configured on this system, or (2) the
configuration wasn't successful.

(1) If it hasn't been configured at all, use the command below to configure
it (set a build directory and let it build its necessary software in it).

      $ ./project configure

(2) If it has been configured, but the configuration failed in a step, you
can re-configure it using your previous settings with the command
below. All successful steps will be skipped, allowing a fast completion.

      $ ./project configure -e

If there was a problem, please let us know by filling this online form:
      http://savannah.nongnu.org/support/?func=additem&group=reproduce

EOF
    exit 1
}





# Run operations in controlled environment
# ----------------------------------------
controlled_env() {

    # Get the full address of the build directory:
    bdir=`.local/bin/realpath .build`

    # Remove all existing environment variables (with 'env -i') and only
    # use some pre-defined environment variables, then build the project.
    envmake=".local/bin/env -i HOME=$bdir sys_rm=$(which rm) $gopt"
    envmake="$envmake separatesupplement=$separatesupplement "
    envmake="$envmake highlightnew=$highlightnew"
    envmake="$envmake highlightnotes=$highlightnotes .local/bin/make "
    envmake="$envmake --no-builtin-rules --no-builtin-variables -f $1"
    if ! [ x"$debug" = x  ]; then envmake="$envmake --debug=$debug"; fi

    # Set the number of jobs. Note that for the 'configure.sh' script the
    # default value has to be 0, so the default is the maximum number of
    # threads. But here, the default value is 1.
    if ! [ x"$jobs"  = x0 ]; then envmake="$envmake -j$jobs";  fi

    # Run the project
    if [ x"$group" = x ]; then
        $envmake $make_targets
    else
        # Set the group and permission flags.
        sg "$group" "umask $perms && $envmake $make_targets"
    fi
}





# Do requested operation
# ----------------------
perms="u+r,u+w,g+r,g+w,o-r,o-w,o-x"
configscript=./reproduce/software/shell/configure.sh
case $operation in

    # Build the project's software.
    configure)

        # Set executable flags
        # --------------------
        #
        # In some scenarios (for example when using a tarball from arXiv),
        # it may happen that the host server has removed the executable
        # flags of all the files. In 'README.md' we instruct the readers on
        # setting the executable flag of this script. But we don't want the
        # user to have to worry about any other file that needs an
        # executable flag.
        #
        # Basically, all the project shell scripts need executable flags so
        # to make sure they have them, we are activating the executable
        # flags by default here every time './project configure' is run. If
        # any other file in your project needs such flags, add them here.
        chmod +x reproduce/software/shell/* reproduce/software/config/*.sh \
              reproduce/analysis/bash/*

        # If the user requested, clean the TeX directory from the extra
        # (to-be-built) directories that may already be there (and will not
        # allow the configuration to complete).
        if [ x"$clean_texdir" = x1 ]; then
            rm -rf tex/build tex/tikz
        fi

        # Variables to pass to the configuration script.
        export jobs=$jobs
        export debug=$debug
        export host_cc=$host_cc
        export build_dir=$build_dir
        export input_dir=$input_dir
        export scriptname=$scriptname
        export maneage_group_name=$group
        export software_dir=$software_dir
        export existing_conf=$existing_conf
        export all_highlevel=$all_highlevel

        # Run the configuration script
        if [ x"$group" = x ]; then
            $configscript
        else
            # Set the group and permission flags.
            sg "$group" "umask $perms && $configscript"

            # Set the group writing permission for everything in the
            # installed software directory. The common build process sets
            # the writing permissions of the installed programs/libraries
            # to '755'. So group members can't write over a file. This
            # creates problems when another group member wants to update
            # the software for example. We thus need to manually add the
            # group writing flag to all installed software files.
            echo "Enabling group writing permission on all installed software..."
            .local/bin/chmod -R g+w .local/;
        fi
        ;;





    # Batch execution of the project.
    make)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Run data preparation phase (optionally build Makefiles with
        # special values for optimizing the main 'top-make.mk'). But note
        # that data preparation is only done automatically the first time
        # the project is built (when '.build/software/preparation-done.mk'
        # doesn't yet exist). After that, if the user wants to re-do the
        # preparation they have to use the '--prepare-redo' option.
        if ! [ -f .build/software/preparation-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-prepare.mk
        fi

        # Run the actual project.
        controlled_env reproduce/analysis/make/top-make.mk

        # Print the number of words (if the user has pdftotext outside of
        # Maneage! For now!!!), AND there actually is a 'paper.pdf' (for
        # example when running './project make clean' there isn't any
        # 'paper.pdf').
        if [ -f paper.pdf ]; then
            if type pdftotext > /dev/null 2>/dev/null; then
                numwords=$(pdftotext paper.pdf && cat paper.txt | wc -w)
                numeff=$(echo $numwords | awk '{print $1-850+500}')
                echo; echo "Number of words in full PDF: $numwords"
                if [ $separatesupplement = 1 ]; then
                    echo "No abstract, and captions (250 for each figure): $numeff"
                fi
                rm paper.txt
            fi
        fi
        ;;


    shell)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Run the project's own shell without inheriting any environment
        # from the host. The 'TERM' environment variable is necessary for
        # tools like some text editors.
        bdir=`.local/bin/realpath .build`
        instdir="$bdir"/software/installed
        .local/bin/env -i \
                       HOME="$bdir" \
                       TERM="$TERM" \
                       CCACHE_DISABLE=1 \
                       PATH="$instdir"/bin \
                       LDFLAGS=-L"$instdir"/lib \
                       SHELL="$instdir"/bin/bash \
                       CPPFLAGS=-I"$instdir"/include \
                       LD_LIBRARY_PATH="$instdir"/lib \
                       OMPI_MCA_plm_rsh_agent=/bin/false \
                       PYTHONPATH="$instdir"/lib/python/site-packages \
                       PYTHONPATH3="$instdir"/lib/python/site-packages \
                       PS1="[\[\033[01;35m\]maneage@\h \W\[\033[32m\]\[\033[00m\]]$ " \
                       "$instdir"/bin/bash
        ;;


    # Operation not specified.
    *)
        cat <<EOF

No operation defined!

Please run with '--help' for more information.
(TIP: available operations are: 'configure', 'make', or 'shell').

EOF
        exit 1
        ;;
esac


==> reproduce/analysis/bash/download-multi-try <==
#!/bin/sh
#
# Attempt downloading multiple times before crashing whole project. From
# the top project directory (for the shebang above), this script must be
# run like this:
#
#   $ /path/to/download-multi-try downloader lockfile input-url downloaded-name
#
# NOTE: The 'downloader' must contain the option to specify the output name
# in its end. For example "wget -O". Any other option can also be placed in
# the middle.
#
# Due to temporary network problems, a download may fail suddenly, but
# succeed in a second try a few seconds later. Without this script that
# temporary glitch in the network will permanently crash the project and
# it can't continue. The job of this script is to be patient and try the
# download multiple times before crashing the whole project.
#
# LOCK FILE: Since there is usually only one network port to the outside
# world, downloading is done much faster in serial, not in parallel. But
# the project's processing may be done in parallel (with multiple threads
# needing to download different files at the same time). Therefore, this
# script uses the 'flock' program to only do one download at a time. To
# benefit from it, any call to this script must be given the same lock
# file. If your system has multiple ports to the internet, or for any
# reason, you don't want to use a lock file, set the 'lockfile' name to
# 'nolock'.
#
# Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.





# Script settings
# ---------------
# Stop the script if there are any errors.
set -e





# Input arguments and necessary sanity checks. Note that the 5th argument
# (backup servers) isn't mandatory.
inurl="$3"
outname="$4"
lockfile="$2"
downloader="$1"
backupservers="$5"
if [ "x$downloader" = x ]; then
    echo "$0: downloader (first argument) not given."; exit 1;
fi
if [ "x$lockfile" = x ]; then
    echo "$0: lock file (second argument) not given."; exit 1;
fi
if [ "x$inurl" = x ]; then
    echo "$0: full input URL (third argument) not given."; exit 1;
fi
if [ "x$outname" = x ]; then
    echo "$0: output name (fourth argument) not given."; exit 1;
fi





# Separate the actual filename, to possibly use backup server.
urlfile=$(echo "$inurl" | awk -F "/" '{print $NF}')





# Try downloading multiple times before crashing.
counter=0
maxcounter=10
while [ ! -f "$outname" ]; do

    # Increment the counter.
    counter=$(echo $counter | awk '{print $1+1}')

    # If we have passed a maximum number of trials, just exit with
    # a failed code.
    reachedmax=$(echo $counter \
         | awk '{if($1>'$maxcounter') print "yes"; else print "no";}')
    if [ x$reachedmax = xyes ]; then
        echo ""
	echo "Failed $maxcounter download attempts: $outname"
        echo ""
	exit 1
    fi

    # If this isn't the first attempt print a notice and wait a little for
    # the next trail.
    if [ x$counter = x1 ]; then
        just_a_place_holder=1
    else
        tstep=$(echo $counter | awk '{print $1*5}')
        echo "Download trial $counter for '$outname' in $tstep seconds."
        sleep $tstep
    fi

    # Attempt downloading the file. Note that the 'downloader' ends with
    # the respective option to specify the output name. For example "wget
    # -O" (so 'outname', that comes after it) will be the name of the
    # downloaded file.
    if [ x"$lockfile" = xnolock ]; then
        if ! $downloader $outname $inurl; then rm -f $outname; fi
    else
        # Try downloading from the requested URL.
        flock "$lockfile" sh -c \
              "if ! $downloader $outname $inurl; then rm -f $outname; fi"
    fi

    # If the download failed, try the backup server(s).
    if [ ! -f "$outname" ]; then
        if [ x"$backupservers" != x ]; then
            for bs in $backupservers; do

                # Use this backup server.
                if [ x"$lockfile" = xnolock ]; then
                    if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi
                else
                    flock "$lockfile" sh -c \
                          "if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi"
                fi

                # If the file was downloaded, break out of the loop that
                # parses over the backup servers.
                if [ -f "$outname" ]; then break; fi
            done
        fi
    fi
done





# Return successfully
exit 0


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
	doi = {10.1088/0004-6256/139/5/1782},
	url = {https://doi.org/10.1088%2F0004-6256%2F139%2F5%2F1782},
	year = 2010,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {139},
	number = {5},
	pages = {1782},
	author = {Dustin Lang and David W. Hogg and Keir Mierle and Michael Blanton and Sam Roweis},
	title = {{ASTROMETRY}.{NET}: {BLIND} {ASTROMETRIC} {CALIBRATION} {OF} {ARBITRARY} {ASTRONOMICAL} {IMAGES}},
	journal = {AJ}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {JOSS},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
   author = {{Behnel}, S. and {Bradshaw}, R. and {Citro}, C. and {Dalcin}, L. and
	{Seljebotn}, D.~S. and {Smith}, K.},
    title = "{Cython: The Best of Both Worlds}",
  journal = {CiSE},
     year = 2011,
    month = mar,
   volume = 13,
   number = 2,
    pages = {31},
      doi = {10.1109/MCSE.2010.118},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astron.Comput.},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
   author = {{Akhlaghi}, M. and {Ichikawa}, T.},
    title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1505.01664},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric},
     year = 2015,
    month = sep,
   volume = 220,
      eid = {1},
    pages = {1},
      doi = {10.1088/0067-0049/220/1/1},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wand
        elt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = "2005",
        month = "Apr",
       volume = {622},
       number = {2},
        pages = {759},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
   author = {{Erwin}, P.},
    title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1408.1097},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric },
     year = 2015,
    month = feb,
   volume = 799,
      eid = {226},
    pages = {226},
      doi = {10.1088/0004-637X/799/2/226},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@Article{matplotlib2007,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {CiSE},
  Volume    = {9},
  Number    = {3},
  Pages     = {90},
  publisher = {IEEE COMPUTER SOC},
  doi       = {10.1109/MCSE.2007.55},
  year      = 2007
}


==> reproduce/software/bibtex/missfits.tex <==
%% Copyright (C) 2020-2022 Surena Fatemi <surena.fatemi@ipm.ir>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{missfits,
       author = {{Marmo}, C. and {Bertin}, E.},
        title = "{MissFITS and WeightWatcher: Two Optimised Tools for Managing FITS Data.}",
      journal = {ASPC},
         year = 2008,
       volume = {394},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {619},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ASPC..394..619M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
   author = {{Dalcin}, L.~D. and {Paz}, R.~R. and {Kler}, P.~A. and {Cosimo}, A.
	},
    title = "{Parallel distributed computing using Python}",
  journal = {AdvWatRes},
     year = 2011,
    month = sep,
   volume = 34,
    pages = {1124},
      doi = {10.1016/j.advwatres.2011.04.013},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2011,
   author = {{van der Walt}, S. and {Colbert}, S.~C. and {Varoquaux}, G.},
    title = "{The NumPy Array: A Structure for Efficient Numerical Computation}",
  journal = {CiSE},
archivePrefix = "arXiv",
   eprint = {1102.1523},
 primaryClass = "cs.MS",
     year = 2011,
    month = mar,
   volume = 13,
   number = 2,
    pages = {22},
      doi = {10.1109/MCSE.2011.37},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011CSE....13b..22V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/r-cran.tex <==
%% Copyright (C) 2022 Boud Roukema <boud@cosmo.torun.pl>
%% Copyright (C) 2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{RIhakaGentleman1996,
      author = {{Ihaka}, Ross and {Gentleman}, Robert},
       title = "{R: A language for data analysis and graphics}",
     journal = {J.Comput.Graph.Stat.},
        year = {1996},
      volume = {5},
      number = {3},
       pages = {299-314},
         DOI = {10.1080/10618600.1996.10474713},
        ISSN = {10618600},
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2011,
   author = {K. J. {Millman} and M. {Aivazis}},
  journal = {CiSE},
    title = {Python for Scientists and Engineers},
     year = {2011},
   volume = {13},
   number = {2},
    pages = {9},
 keywords = {Special issues and sections;Computer languages;Programming;Scientific computing;Numerical models;Programming languages;Python;Scientific computing;interactive research;Python libraries;Python tools},
      doi = {10.1109/MCSE.2011.36},
     ISSN = {1521-9615},
    month ={March},
}

@ARTICLE{scipy2007,
   author = {T. E. {Oliphant}},
  journal = {CiSE},
    title = {Python for Scientific Computing},
     year = {2007},
   volume = {9},
   number = {3},
    pages = {10},
 keywords = {high level languages;Python;scientific computing;steering language;scientific codes;high-level language;Scientific computing;High level languages;Libraries;Writing;Application software;Embedded software;Software standards;Standards development;Internet;Prototypes;Python;computer languages;scientific programming;scientific computing},
      doi = {10.1109/MCSE.2007.58},
     ISSN = {1521-9615},
    month = {May},
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = "1996",
        month = "Jun",
       volume = {117},
        pages = {393},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019-2022 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {5:1},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}


==> reproduce/software/shell/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the 'MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/shell/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the 'MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> tex/build/macros/dependencies-bib.tex <==



==> tex/src/figure-data-lineage.tex <==
% All macros commented                %  1
\newcommand{\paperpdf}{}              %  2
\newcommand{\papertex}{}              %  3
\newcommand{\projecttex}{}            %  4
\newcommand{\verifytex}{}             %  5
\newcommand{\initializetex}{}         %  6
\newcommand{\demoplottex}{}           %  7
\newcommand{\toolsperyear}{}          %  8
\newcommand{\tablethree}{}            %  9
\newcommand{\menkexlsx}{}             % 10
\newcommand{\inputsconf}{}            % 11
\newcommand{\downloadtex}{}           % 12
\newcommand{\formattex}{}             % 13
\newcommand{\demoyearconf}{}          % 14
\newcommand{\expandingproject}{}      % 15





%% Start the TiKZ picture environment.
\begin{tikzpicture}[
  line width=1.5pt,
  black!50,
  text=black,
]

  %% Use small fonts
  \footnotesize

  %% These white lines are only relevant when we want to add boxes in
  %% multiple figures (for example to build slides). They are used to fix
  %% the vertical position of the boxs in the figure so it doesn't change
  %% as we add more boxes.
  \draw [white] (-7.6,0) -- (7.5,0);
  \draw [white] (0,-4.5) -- (0,4.9);

  %% top-make.mk
  \node [at={(-0.05cm,2mm)},
         rectangle,
         very thick,
         text centered,
         font=\ttfamily,
         text width=2.8cm,
         minimum width=15cm,
         minimum height=7.8cm,
         draw=green!50!black!50,
         fill=black!10!green!2!white,
         label={[shift={(0,-5mm)}]\texttt{top-make.mk}}] {};

  %% Work-horse Makefiles. -5.6 -> -5.73 = -0.13
  \node (initializemk) [node-makefile, at={(-5.73cm,-1.3cm)},
    label={[shift={(0,-5mm)}]\texttt{initialize.mk}}] {};
  \node (downloadmk)   [node-makefile, at={(-2.93cm,-1.3cm)},
    label={[shift={(0,-5mm)}]\texttt{download.mk}}] {};
  \node (analysis1mk)  [node-makefile, at={(-0.13cm,-1.3cm)},
    label={[shift={(0,-5mm)}]\texttt{format.mk}}] {};
  \node (analysis2mk)  [node-makefile, at={(2.67cm,-1.3cm)},
    label={[shift={(0,-5mm)}]\texttt{demo-plot.mk}}] {};

  %% verify.mk
  \node [at={(-5.3cm,-2.8cm)},
         thick,
         rectangle,
         text centered,
         font=\ttfamily,
         text width=2.45cm,
         minimum width=3.5cm,
         minimum height=1.3cm,
         draw=green!50!black!50,
         fill=black!10!green!12!white,
         label={[shift={(1cm,-5mm)}]\texttt{verify.mk}}] {};

  %% Paper.mk
  \node [at={(2.67cm,-2.8cm)},
         thick,
         rectangle,
         text centered,
         text width=2.8cm,
         minimum width=8.5cm,
         minimum height=1.3cm,
         draw=green!50!black!50,
         fill=black!10!green!12!white,
         font=\ttfamily,
         label={[shift={(0,-5mm)}]\texttt{paper.mk}}] {};

  %% paper.pdf
  \ifdefined\paperpdf
  \node (paperpdf) [node-terminal, at={(5.47cm,-2.9cm)}] {paper.pdf};
  \fi

  %% paper.tex
  \ifdefined\papertex
  \node (reftex) [node-nonterminal, at={(2.67cm,-4.2cm)}] {references.tex};
  \node (papertex) [node-nonterminal, at={(5.47cm,-4.2cm)}] {paper.tex};
  \node (papertex-north) [node-point, at={(5.47cm,-3.58cm)}] {};
  \draw [rounded corners] (reftex) |- (papertex-north);
  \draw [->] (papertex) -- (paperpdf);
  \fi

  %% project.tex
  \ifdefined\projecttex
  \node (projecttex) [node-terminal, at={(-0.13cm,-2.9cm)}] {project.tex};
  \draw [->] (projecttex) -- (paperpdf);
  \fi

  %% verify.tex
  \ifdefined\verifytex
  \node (verifytex) [node-terminal, at={(-5.73cm,-2.9cm)}] {verify.tex};
  \draw [->] (verifytex) -- (projecttex);
  \fi

  %% Initialize.tex
  \ifdefined\initializetex
  \node (initializetex) [node-terminal, at={(-5.73cm,-0.8cm)}] {initialize.tex};
  \node (initialize-south) [node-point, at={(-5.73cm,-1.5cm)}] {};
  \draw [->] (initializetex) -- (verifytex);
  \node [anchor=west, at={(-7.05cm,2.30cm)}] {Basic project info};
  \node [anchor=west, at={(-7.05cm,1.95cm)}] {(e.g., Git commit).};
  \node [anchor=west, at={(-7.05cm,1.10cm)}] {Also defines};
  \node [anchor=west, at={(-7.05cm,0.75cm)}] {project structure};
  \node [anchor=west, at={(-7.05cm,0.40cm)}] {(for \texttt{*.mk} files).};
  \fi

  %% demo-plot.tex
  \ifdefined\demoplottex
  \node (dptex) [node-terminal, at={(2.67cm,-0.8cm)}] {demo-plot.tex};
  \draw [rounded corners, -] (dptex) |- (initialize-south);
  \fi

  %% tools-per-year.txt
  \ifdefined\toolsperyear
  \node (tpyear) [node-terminal, at={(2.67cm,0.3cm)}] {tools-per-\\year.txt};
  \draw [->] (tpyear) -- (dptex);
  \fi

  %% table-3.txt
  \ifdefined\tablethree
  \node (tabthree) [node-terminal, at={(-0.13cm,1.1cm)}] {table-3.txt};
  \draw [rounded corners, ->] (tabthree) |- (tpyear);
  \fi

  %% menkexlsx
  \ifdefined\menkexlsx
  \node (xlsx) [node-terminal, at={(-2.93cm,1.9cm)}] {menke20.xlsx};
  \draw [->, rounded corners] (xlsx) |- (tabthree);
  \fi

  %% INPUTS.conf
  \ifdefined\inputsconf
  \node (INPUTS) [node-nonterminal, at={(-2.93cm,4.6cm)}] {INPUTS.conf};
  \node (xlsx-west) [node-point, at={(-4.33cm,1.9cm)}] {};
  \draw [->,rounded corners] (INPUTS.west) -| (xlsx-west) |- (xlsx);
  \fi

  %% download.tex
  \ifdefined\downloadtex
  \node (downloadtex) [node-terminal, at={(-2.93cm,-0.8cm)}] {download.tex};
  \node (downloadtex-west) [node-point, at={(-4.33cm,-0.8cm)}] {};
  \draw [->,rounded corners] (INPUTS.west) -| (downloadtex-west)
                             |- (downloadtex);
  \draw [rounded corners, -] (downloadtex) |- (initialize-south);
  \fi

  %% format.tex
  \ifdefined\formattex
  \node (fmttex) [node-terminal, at={(-0.13cm,-0.8cm)}] {format.tex};
  \draw [->] (tabthree) -- (fmttex);
  \draw [rounded corners, -] (fmttex) |- (initialize-south);
  \fi

  %% demo-year.conf
  \ifdefined\demoyearconf
  \node (dyearconf) [node-nonterminal, at={(2.67cm,4.6cm)}] {demo-year.conf};
  \node (dptex-west) [node-point, at={(1.27cm,-0.8cm)}] {};
  \draw [->,rounded corners] (dyearconf.west) -| (dptex-west) |- (dptex);
  \fi

  %% Expanding project
  \ifdefined\expandingproject

    %% The Makefile.
    \node [opacity=0.7, dashed] (analysis3mk)  [node-makefile, at={(5.47cm,-1.3cm)},
      label={[shift={(0,-5mm)}, opacity=0.7]\texttt{next-step.mk}}] {};

    %% next-step.tex
    \node [opacity=0.7, dashed] (a3tex) [node-terminal, at={(5.47cm,-0.8cm)}] {next-step.tex};
    \draw [opacity=0.7, rounded corners, -, dashed] (a3tex) |- (initialize-south);

    % out-3a.dat and out-3b.dat
    \node [opacity=0.7, dashed] (out3a) [node-terminal, at={(5.47cm,2.7cm)}] {out-a.dat};
    \node [opacity=0.7, dashed] (out3b) [node-terminal, at={(5.47cm,1.1cm)}] {out-b.dat};
    \node (a3tex-east) [node-point, at={(6.87cm,-0.8cm)}] {};
    \draw [opacity=0.7, ->,rounded corners, dashed] (out3a.east) -| (a3tex-east) |- (a3tex);
    \draw [opacity=0.7, ->, dashed] (out3b) -- (a3tex);

    %% demo-out.dat
    \node [opacity=0.7, dashed] (dout) [node-terminal, at={(2.67cm,1.9cm)}] {demo-out.dat};
    \draw [opacity=0.7, ->, rounded corners, dashed] (dout.south) |- (out3b);

    %% links
    \node (dout-west) [node-point, at={(1.27cm,1.9cm)}] {};
    \draw [opacity=0.7, ->, dashed] (xlsx) -- (dout);
    \node [opacity=0.7] (out3a-west) [node-point, at={(4.07cm,2.7cm)}] {};
    \draw [opacity=0.7, ->,rounded corners, dashed] (xlsx) |- (out3a);
    \node [opacity=0.7, dashed] (a3conf1) [node-nonterminal, at={(5.47cm,4.6cm)}]  {param.conf};
    \draw [opacity=0.7, rounded corners, dashed] (a3conf1.west) -| (out3a-west) |- (out3a);
  \fi
\end{tikzpicture}


==> tex/src/figure-file-architecture.tex <==
\newcommand{\fullfilearchitecture}{}

\begin{tikzpicture}[
  line width=1.5pt,
  black!50,
  text=black,
]

  %% Use small fonts
  \footnotesize

  %% project/
  \node [dirbox, at={(0,4cm)}, minimum width=15cm, minimum height=9.9cm,
    label={[shift={(0,-5mm)}]\texttt{project/}}] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-6.0cm,3.3cm)}] {COPYING};
  \fi
  \node [node-nonterminal-thin, at={(-3.5cm,3.3cm)}] {paper.tex};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-1.0cm,3.3cm)}] {project};
  \node [node-nonterminal-thin, at={(+1.5cm,3.3cm)}] {README.md};
  \node [node-nonterminal-thin, at={(+4.25cm,3.3cm)},
    text width=2.5cm, text depth=-3pt] {README-hacking.md};
  \fi

  %% reproduce/
  \node [dirbox, at={(-1.4cm,2.6cm)}, minimum width=11.9cm, minimum height=6cm,
    label={[shift={(0,-5mm)}]\texttt{reproduce/}}, fill=brown!15!white] {};

  %% reproduce/software/
  \node [dirbox, at={(-4.35cm,2.1cm)}, minimum width=5.7cm, minimum height=5.3cm,
    label={[shift={(0,-5mm)}]\texttt{software/}}, fill=brown!20!white] {};

  %% reproduce/software/config/
  \node [dirbox, at={(-5.75cm,1.5cm)}, minimum width=2.6cm, minimum height=2.1cm,
    label={[shift={(0,-5mm)}]\texttt{config/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-5.75cm,0.8cm)}] {TARGETS.conf};
  \fi
  \node [node-nonterminal-thin, at={(-5.75cm,0.3cm)}] {versions.conf};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-5.75cm,-0.2cm)}] {checksums.conf};
  \fi

  %% reproduce/software/make/
  \node [dirbox, at={(-2.95cm,1.5cm)}, minimum width=2.6cm, minimum height=2.1cm,
    label={[shift={(0,-5mm)}]\texttt{make/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-2.95cm,0.8cm)}] {basic.mk};
  \fi
  \node [node-nonterminal-thin, at={(-2.95cm,0.3cm)}] {high-level.mk};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-2.95cm,-0.2cm)}] {python.mk};
  \fi

  %% reproduce/software/bash/
  \node [dirbox, at={(-5.75cm,-0.8cm)}, minimum width=2.6cm, minimum height=1.6cm,
    label={[shift={(0,-5mm)}]\texttt{shell/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-5.75cm,-1.5cm)}] {configure.sh};
  \node [node-nonterminal-thin, at={(-5.75cm,-2.0cm)}] {bashrc.sh};
  \fi

  %% reproduce/software/bibtex/
  \node [dirbox, at={(-2.95cm,-0.8cm)}, minimum width=2.6cm, minimum height=2.1cm,
    label={[shift={(0,-5mm)}]\texttt{bibtex/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(-2.95cm,-1.5cm)}] {fftw.tex};
  \node [node-nonterminal-thin, at={(-2.95cm,-2.0cm)}] {numpy.tex};
  \node [node-nonterminal-thin, at={(-2.95cm,-2.5cm)}] {gnuastro.tex};
  \fi

  %% reproduce/analysis/
  \node [dirbox, at={(1.55cm,2.1cm)}, minimum width=5.7cm, minimum height=5.3cm,
    label={[shift={(0,-5mm)}]\texttt{analysis/}}, fill=brown!20!white] {};

  %% reproduce/analysis/config/
  \node [dirbox, at={(0.15cm,1.5cm)}, minimum width=2.6cm, minimum height=2.6cm,
    label={[shift={(0,-5mm)}]\texttt{config/}}, fill=brown!25!white] {};
  \node [node-nonterminal-thin, at={(0.15cm,0.8cm)}] {INPUTS.conf};
  \node [node-nonterminal-thin, at={(0.15cm,0.3cm)}] {param-1.conf};
  \node [node-nonterminal-thin, at={(0.15cm,-0.2cm)}] {param-2a.conf};
  \node [node-nonterminal-thin, at={(0.15cm,-0.7cm)}] {param-2b.conf};

  %% reproduce/analysis/make/
  \node [dirbox, at={(2.95cm,1.5cm)}, minimum width=2.6cm, minimum height=2.6cm,
    label={[shift={(0,-5mm)}]\texttt{make/}}, fill=brown!25!white] {};
  \node [node-nonterminal-thin, at={(2.95cm,0.8cm)}] {top-prepare.mk};
  \node [node-nonterminal-thin, at={(2.95cm,0.3cm)}] {top-make.mk};
  \node [node-nonterminal-thin, at={(2.95cm,-0.2cm)}] {initialize.mk};
  \node [node-nonterminal-thin, at={(2.95cm,-0.7cm)}] {format.mk};

  %% reproduce/analysis/bash/
  \node [dirbox, at={(0.15cm,-1.3cm)}, minimum width=2.6cm, minimum height=1.1cm,
    label={[shift={(0,-5mm)}]\texttt{bash/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(0.15cm,-2.0cm)}] {process-A.sh};
  \fi

  %% reproduce/analysis/python/
  \node [dirbox, at={(2.95cm,-1.3cm)}, minimum width=2.6cm, minimum height=1.6cm,
    label={[shift={(0,-5mm)}]\texttt{python/}}, fill=brown!25!white] {};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(2.95cm,-2.0cm)}] {operation-B.py};
  \node [node-nonterminal-thin, at={(2.95cm,-2.5cm)}] {fitting-plot.py};
  \fi

  %% tex/
  \node [dirbox, at={(6cm,2.6cm)}, minimum width=2.7cm, minimum height=6cm,
    label={[shift={(0,-5mm)}]\texttt{tex/}}, fill=brown!15!white] {};

  %% tex/src/
  \node [dirbox, at={(6cm,2.1cm)}, minimum width=2.5cm, minimum height=1.6cm,
    label={[shift={(0,-5mm)}]\texttt{src/}}, fill=brown!20!white] {};
  \node [node-nonterminal-thin, at={(6cm,1.4cm)}] {references.tex};
  \ifdefined\fullfilearchitecture
  \node [node-nonterminal-thin, at={(6cm,0.9cm)}] {figure-1.tex};
  \fi

  %% tex/build/
  \ifdefined\fullfilearchitecture
  \node [dirbox, at={(6cm,0.1cm)}, minimum width=2.5cm, minimum height=1.3cm,
    label={[shift={(0,-5mm)}]\texttt{build/}}, dashed, , fill=brown!20!white] {};
  \node [anchor=west, at={(4.7cm,-0.7cm)}] {\scriptsize\sf Symbolic link to};
  \node [anchor=west, at={(4.7cm,-1.0cm)}] {\scriptsize\sf \LaTeX{} build directory.};
  \fi

  %% tex/tikz/
  \ifdefined\fullfilearchitecture
  \node [dirbox, at={(6cm,-1.6cm)}, minimum width=2.5cm, minimum height=1.6cm,
    label={[shift={(0,-5mm)}]\texttt{tikz/}}, dashed, fill=brown!20!white] {};
  \node [anchor=west, at={(4.67cm,-2.4cm)}] {\scriptsize\sf Symbolic link to TikZ};
  \node [anchor=west, at={(4.67cm,-2.7cm)}] {\scriptsize\sf directory (figures built};
  \node [anchor=west, at={(4.67cm,-3.0cm)}] {\scriptsize\sf by \LaTeX).};
  \fi

  %% .git/
  \ifdefined\fullfilearchitecture
  \node [dirbox, at={(0,-3.6cm)}, minimum width=14.2cm, minimum height=7mm,
    label={[shift={(0,-5mm)}]\texttt{.git/}}, fill=brown!15!white] {};
  \node [anchor=north, at={(0cm,-3.9cm)}]
        {\scriptsize\sf Full project temporal provenance (version controlled history) in Git.};
  \fi

  %% .local/
  \ifdefined\fullfilearchitecture
  \node [dirbox, at={(-3.6cm,-4.5cm)}, minimum width=7cm, minimum height=1.2cm,
    label={[shift={(0,-5mm)}]\texttt{.local/}}, dashed, fill=brown!15!white] {};
  \node [anchor=west, at={(-7.1cm,-5.2cm)}]
        {\scriptsize\sf Symbolic link to project's software environment, e.g., };
  \node [anchor=west, at={(-7.1cm,-5.5cm)}]
        {\scriptsize\sf Python or R, run `\texttt{.local/bin/python}' or `\texttt{.local/bin/R}'};
  \fi

  %% .build/
  \ifdefined\fullfilearchitecture
  \node [dirbox, at={(3.6cm,-4.5cm)}, minimum width=7cm, minimum height=1.2cm,
    label={[shift={(0,-5mm)}]\texttt{.build/}}, dashed, fill=brown!15!white] {};
  \node [anchor=west, at={(0.1cm,-5.2cm)}]
        {\scriptsize\sf Symbolic link to project's top-level build directory.};
  \node [anchor=west, at={(0.1cm,-5.5cm)}]
        {\scriptsize\sf Enabling easy access to all of project's built components.};
  \fi

\end{tikzpicture}


==> tex/src/figure-project-outline.tex <==
% Copyright (C) 2018-2022 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
% This LaTeX source is free software: you can redistribute it and/or
% modify it under the terms of the GNU General Public License as
% published by the Free Software Foundation, either version 3 of the
% License, or (at your option) any later version.
%
% This LaTeX source is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
% General Public License for more details.
%
% You should have received a copy of the GNU General Public License
% along with this LaTeX source.  If not, see <https://www.gnu.org/licenses/>.

%% Environment variables.
\newcommand{\allopacity}{1}
\newcommand{\sver}{}
\newcommand{\srep}{}
\newcommand{\dver}{}
\newcommand{\ddver}{}
\newcommand{\confopt}{}
\newcommand{\confenv}{}
\newcommand{\containers}{}
\newcommand{\db}{}
\newcommand{\calib}{}
\newcommand{\corr}{}
\newcommand{\runord}{}
\newcommand{\runopt}{}
\newcommand{\humanerr}{}
\newcommand{\confirmbias}{}
\newcommand{\depupdate}{}
\newcommand{\coauth}{}
\newcommand{\varsinpaper}{}
\newcommand{\recordinfo}{}
\newcommand{\softcite}{}
\newcommand{\prevchange}{}

\begin{tikzpicture}[>=stealth, thick, black!50, text=black,
    every new ->/.style={shorten >=1pt},
    hv path/.style={to path={-| (\tikztotarget)}},
    graphs/every graph/.style={edges=rounded corners}]

    \footnotesize

  %% This white line is only added to fix the vertical position of the
  %% figure so it doesn't change as we add more boxes.
  \draw [white] (0,-4.3) -- (0,3.8);
  \draw [white] (-0.5,0) -- (12,0);

  %% Box showing containers.
  \ifdefined\containers
    \filldraw[orange!20!white, rounded corners=2mm] (-0.1,0.3) rectangle (5.6,3.8);
    \draw (-0.1,3.65) node [anchor=west] {\scriptsize Existing solutions:};
    \draw (0,3.35) node [anchor=west] {\scriptsize Virtual machines};
    \draw (0,3.05) node [anchor=west] {\scriptsize Containers};
    \draw (0,2.75) node [anchor=west] {\scriptsize Package managers};
  \fi

  \graph[grow right sep, simple] {
    { [nodes={yshift=7mm}]
      soft/Software [gbox] -> build/Build [bbox],
      hard/Hardware/data [gbox, yshift=-0.5cm] --
      p1 [coordinate, xshift=2cm, yshift=-0.5cm]
    } -- [hv path]
    p2 [coordinate] ->
    srun/Run software on data [bbox] ->
    paper/Paper [bbox]
  };

  \ifdefined\paperfinal
    \node (happy) [inner sep=0pt, below=of paper, yshift=+8mm]
          {\includegraphics[width=2cm]{img/happy-question.jpg}};
    \node (happyurl) [below=of happy, xshift=-9.5mm, yshift=+1cm]
          {\tiny \url{https://heywhatwhatdidyousay.wordpress.com}};
    \node (qurl) [below=of happyurl, xshift=10.5mm, yshift=+1.2cm]
          {\tiny \url{http://pngimages.net}};
  \else
    \ifdefined\paperinit
      \node (happy) [inner sep=0pt, below=of paper, yshift=+8mm]
            {\includegraphics[width=2cm]{img/happy.jpg}};
      \node (happyurl) [below=of happy, xshift=-9.5mm, yshift=+1cm]
            {\tiny \url{https://heywhatwhatdidyousay.wordpress.com}};
    \fi
  \fi

  %% Software...
  \let\ppopacity\undefined
  \ifdefined\allopacity \newcommand{\ppopacity}{1}
  \else \ifdefined\focusonpackages
      \newcommand{\ppopacity}{1}
    \else
      \newcommand{\ppopacity}{0.3}
    \fi
  \fi

  \ifdefined\sver
  \node (sver)
        [rbox, above=of soft, yshift=-8mm, opacity=\ppopacity]
        {What version?};
  \fi
  \ifdefined\srep
  \node (srep)
        [rbox, above=of sver, yshift=-8mm, opacity=\ppopacity]
        {Repository?};
  \fi

  %% Build
  \ifdefined\dver
  \node (dver)
        [rbox, above=of build, yshift=-8mm, opacity=\ppopacity]
        {Dependencies?};
  \fi
  \ifdefined\ddver
  \node (ddver)
        [rbox, above=of dver, yshift=-8mm, opacity=\ppopacity]
        {Dep. versions?};
  \fi
  \ifdefined\confopt
  \node (confopt)
        [rbox, above=of ddver, yshift=-8mm, opacity=\ppopacity]
        {Config options?};
  \fi
  \ifdefined\confenv
  \node (confenv)
        [rbox, above=of confopt, yshift=-8mm, opacity=\ppopacity]
        {Config environment?};
  \fi

  %% Hardware/data
  \let\ppopacity\undefined
  \ifdefined\allopacity \newcommand{\ppopacity}{1}
  \else \ifdefined\focusonhardware
      \newcommand{\ppopacity}{1}
    \else
      \newcommand{\ppopacity}{0.3}
    \fi
  \fi
  \ifdefined\db
  \node (db)
        [rbox, below=of hard, yshift=+8mm, opacity=\ppopacity]
        {Data base, or PID?};
  \fi
  \ifdefined\calib
  \node (calib)
        [rbox, below=of db, yshift=+8mm, opacity=\ppopacity]
        {Calibration/version?};
  \fi
  \ifdefined\corr
  \node (corr)
        [rbox, below=of calib, yshift=+8mm, opacity=\ppopacity]
        {Integrity?};
  \fi

  %% Run software ...
  \let\ppopacity\undefined
  \ifdefined\allopacity \newcommand{\ppopacity}{1}
  \else \ifdefined\focusonrun
      \newcommand{\ppopacity}{1}
    \else
      \newcommand{\ppopacity}{0.3}
    \fi
  \fi
  \ifdefined\runord
  \node (runord)
        [rbox, above=of srun, yshift=-8mm, opacity=\ppopacity]
        {What order?};
  \fi
  \ifdefined\runopt
  \node (runopt)
        [rbox, above=of runord, yshift=-8mm, opacity=\ppopacity]
        {Runtime options?};
  \fi
  \ifdefined\humanerr
  \node (humanerr)
        [rbox, above=of runopt, yshift=-8mm, opacity=\ppopacity]
        {Human error?};
  \fi
  \ifdefined\confirmbias
  \node (confirmbias)
        [rbox, above=of humanerr, yshift=-8mm, opacity=\ppopacity]
        {Confirmation bias?};
  \fi
  \ifdefined\depupdate
  \node (depupdate)
        [rbox, below=of srun, yshift=+8mm, opacity=\ppopacity]
        {Environment update?};
  \fi
  \ifdefined\coauth
  \node (coaut)
        [rbox, below=of depupdate, yshift=+8mm, opacity=\ppopacity]
        {In sync with coauthors?};
  \fi

  %% Paper ...
  \let\ppopacity\undefined
  \ifdefined\allopacity \newcommand{\ppopacity}{1}
  \else \ifdefined\focusonpaper
      \newcommand{\ppopacity}{1}
    \else
      \newcommand{\ppopacity}{0.3}
    \fi
  \fi
  \ifdefined\varsinpaper
  \node (varsinpaper)
        [rbox, above=of paper, xshift=-1mm, yshift=-8mm, opacity=\ppopacity]
        {Sync with analysis?};
  \fi
  \ifdefined\recordinfo
  \node (recordinfo)
        [rbox, above=of varsinpaper, yshift=-8mm, opacity=\ppopacity]
        {Report this info?};
  \fi
  \ifdefined\softcite
  \node (softcite)
        [rbox, above=of recordinfo, yshift=-8mm, opacity=\ppopacity]
        {Cited software?};
  \fi
  \ifdefined\prevchange
  \node (prevchange)
        [rbox, above=of softcite, yshift=-8mm, opacity=\ppopacity]
        {History recorded?};
  \fi

  \ifdefined\gitlogo
  \node [inner sep=0pt, opacity=0.5] at (5.5,0)
        {\includegraphics[width=10cm]{img/git.png}};
  \fi
\end{tikzpicture}


==> tex/src/figure-src-demoplot.tex <==
\begin{tcolorbox}[title=\inlinecode{\textcolor{white}{demo-plot.mk}}\hfill(Simplified contents)]
  \footnotesize
  \texttt{\mkcomment{1ST MAKE RULE: build the directory hosting the converted table.}}\\
  \texttt{\mkvar{a2dir} = \$(\mkvar{texdir})/tools-per-year}\\
  \texttt{\mktarget{\$(a2dir)}:; \mkprog{mkdir} \$@}

  \vspace{2em}
  \texttt{\mkcomment{2ND MAKE RULE: extract necessary info from raw table.}}\\
  \texttt{\mkvar{a2mk20f1c} = \$(\mkvar{a2dir})/tools-per-year.txt}\\
  \texttt{\mktarget{\$(a2mk20f1c)}: \$(\mkvar{mk20tab3}) | \$(\mkvar{a2dir})}\\
  \texttt{\mktab{}\mkprog{awk} '!/\^{}\#/ \{all[\$\$1]+=\$\$2; id[\$\$1]+=\$\$3;\}} \textbackslash\\
  \texttt{\mktab{}{ }{ }{ }{ }{ }END\{ for(year in all) print year, 100*id[year]/all[year], all[year] \}}' \textbackslash\\
  \texttt{\mktab{}{ }{ }{ }{ }> \$@}

  \vspace{2em}
  \texttt{\mkcomment{3RD MAKE RULE: Main LaTeX macro file for reported values in text.}}\\
  \texttt{\mkvar{pconfdir} = reproduce/analysis/config}\\
  \texttt{\mktarget{\$(mtexdir)/demo-plot.tex}: \$(\mkvar{a2mk20f1c}) \$(\mkvar{pconfdir})/menke-demo-year.conf}

  %% We need an empty line here for the extra space to work.
  \texttt{\recipecomment{First year data were taken (first column of first row).}}\\
  \texttt{\mktab{}v=\$\$(awk 'NR==1\{print \$\$1\}' \$(\mkvar{a2mk20f1c}))}\\
  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand\{\textbackslash{}menkefirstyear\}\{\$\$v\}" > \$@}

  %% We need an empty line here for the extra space to work.
  \texttt{\recipecomment{Number of papers in the demonstration year. The year is defined in}}

  \texttt{\recipecomment{`\$(pconfdir)/menke-demo-year.conf' as `menke-demo-year' and also passed onto LaTeX.}}\\
  \texttt{\mktab{}v=\$\$(awk '\$\$1==\$(\mkvar{menke-demo-year})\{print \$\$3\}' \$(\mkvar{a2mk20f1c}))}\\
  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand\{\textbackslash{}menkenumpapersdemocount\}\{\$\$v\}"{ }>> \$@} \\
  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand\{\textbackslash{}menkenumpapersdemoyear\}\{\$(\mkvar{menke-demo-year})\}"{ }>> \$@}
\end{tcolorbox}


==> tex/src/figure-src-download.tex <==
\begin{tcolorbox}[title=\inlinecode{\textcolor{white}{download.mk}} \hfill\textcolor{white}{(only \LaTeX{} macro's rule)}]
  \footnotesize
  \texttt{\mkcomment{Write download URL into the paper (through a LaTeX macro).}}

  \texttt{\mktarget{\$(mtexdir)/download.tex}: \$(\mkvar{indir})/menke20.xlsx}

  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand{\textbackslash{}menketwentyurl}\{\mktarget{\$(MK20URL)}\}" > \$@}
\end{tcolorbox}


==> tex/src/figure-src-format.tex <==
\begin{tcolorbox}[title=\inlinecode{\textcolor{white}{format.mk}}\hfill(Simplified contents)]
  \footnotesize
  \texttt{\mkcomment{1ST MAKE RULE: build the directory hosting the converted table.}}

  \texttt{\mkvar{a1dir} = \$(\mkvar{BDIR})/format}

  \texttt{\mktarget{\$(a1dir)}:}

  \texttt{\mktab{}\mkprog{mkdir} \$@}

  \vspace{2em}
  \texttt{\mkcomment{2ND MAKE RULE: Convert the XLSX table to a simple plain-text table.}}

  \texttt{\mkvar{mk20tab3} = \$(\mkvar{a1dir})/menke20-table-3.txt}

  \texttt{\mktarget{\$(mk20tab3)}: \$(\mkvar{indir})/menke20.xlsx | \$(\mkvar{a1dir})}

  \texttt{\recipecomment{Call XLSX I/O to convert all the spreadsheets into different CSV files.}}

  \texttt{\recipecomment{We only want the `table-3' spreadsheet, but XLSX I/O does not allow setting its}}

  \texttt{\recipecomment{output filename. For simplicity, let's assume its written in `table-3.csv'.}}

  \texttt{\mktab{}\mkprog{xlsxio\_xlsx2csv} \$<}

  \vspace{0.5em}
  \texttt{\recipecomment{Use GNU AWK to keep the desired columns in space-separated, fixed-width format.}}

  \texttt{\recipecomment{With `FPAT' commas within double quotes are not counted as columns.}}

  \texttt{\mktab{}\mkprog{awk} 'NR>1\{printf("\%-10d\%-10d\%-10d \%s\textbackslash{}n", \$\$2, \$\$3, \$\$(NF-1)*\$\$NF, \$\$1)\}' \textbackslash}

  \texttt{\mktab{}{ }{ }{ }{ }FPAT='([\^{},]+)|("[\^{}"]+")' table-3.csv > \$@}

  \vspace{0.5em}
  \texttt{\recipecomment{Delete the temporary CSV file.}}

  \texttt{\mktab{}\mkprog{rm} table-3.csv}

  \vspace{2em}
  \texttt{\mkcomment{3RD MAKE RULE: Main LaTeX macro file for reported values.}}

  \texttt{\mktarget{\$(mtexdir)/format.tex}: \$(\mkvar{mk20tab3)}}

  \texttt{\recipecomment{Count the total number of papers in their study to report in this paper.}}

  \texttt{\mktab{}v=\$\$(\mkprog{awk} '\!/\^{}\#/\{c+=\$\$2\} END\{print c\}' \$(\mkvar{mk20tab3)})}

  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand\{\textbackslash{}menkenumpapers\}\{\$\$v\}" > \$@}

  \vspace{0.5em}
  \texttt{\recipecomment{Count total number of journals in that study.}}

  \texttt{\mktab{}v=\$\$(awk 'BEGIN{FIELDWIDTHS="31 10000"} !/\^\#/\{print \$\$2\}' \$(mk20tab3) \textbackslash}

  \texttt{\mktab{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }| uniq | wc -l)}

  \texttt{\mktab{}\mkprog{echo} "\textbackslash{}newcommand\{\textbackslash{}menkenumjournals\}\{\$\$v\}" >> \$@}
\end{tcolorbox}


==> tex/src/figure-src-inputconf.tex <==
\begin{tcolorbox}[title=\inlinecode{\textcolor{white}{INPUT.conf}}]
  \footnotesize
  \texttt{\mkvar{INPUT-{\menketwentyxlsxname}-sha256} = \menketwentychecksum}\\
  \texttt{\mkvar{INPUT-{\menketwentyxlsxname}-size} = \menketwentybytesize}\\
  \texttt{\mkvar{INPUT-{\menketwentyxlsxname}-url} = {\scriptsize \menketwentyurl}}\\
  \vspace{-3mm}
\end{tcolorbox}


==> tex/src/figure-src-topmake.tex <==
\begin{tcolorbox}[title=\inlinecode{\textcolor{white}{top-make.mk}}\hfill\textcolor{white}{(simplified)}]
  \footnotesize

  \texttt{\mkcomment{Ultimate target/purpose of project (`paper.pdf' is the final target of the final subMakefile}}\par
  \texttt{\mkcomment{that is loaded/included below)}}\par
  \texttt{\mktarget{all}: paper.pdf}

  \vspace{1em}
  \texttt{\mkcomment{List of subMakefiles to be loaded in order.}}\par
  \texttt{\mkvar{makesrc} = initialize \textbackslash}\par
  \texttt{{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }download \textbackslash}\par
  \texttt{{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }format \textbackslash}\par
  \texttt{{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }demo-plot \textbackslash}\par
  \texttt{{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }verify \textbackslash}\par
  \texttt{{ }{ }{ }{ }{ }{ }{ }{ }{ }{ }paper}\par

  \vspace{1em}
  \texttt{\mkcomment{Include all the configuration files.}}\par
  \texttt{\textcolor{purple}{include} reproduce/analysis/config/*.conf}

  \vspace{1em}
  \texttt{\mkcomment{Include the subMakefiles in the specified order.}}\par
  \texttt{\textcolor{purple}{include} \$(\textcolor{blue}{foreach} s, \$(\mkvar{makesrc}), reproduce/analysis/make/\$(\mkvar{s}).mk)}
\end{tcolorbox}


==> tex/src/references.tex <==
%% Non-software BibTeX entries. The software-specific BibTeX entries are
%% stored in a `*.tex' file under the `tex/dependencies' directory.
%
%% [[[BibTeX 0.99d complains with the at-character, even when its in a
%%    comment line! So ::at:: is used instead in the email address]]].
%% Copyright (C) 2018-2022 Mohammad Akhlaghi <mohammad::at::akhlaghi.org>
%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.





@ARTICLE{peper20,
       author = {{Peper}, Marius and {Roukema}, Boudewijn F.},
        title = "{The role of the elaphrocentre in low surface brightness galaxy formation}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = oct,
          eid = {arXiv:2010.03742},
        pages = {arXiv:2010.03742},
archivePrefix = {arXiv},
       eprint = {2010.03742},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201003742P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{roukema20,
       author = {{Roukema}, Boudewijn F.},
        title = "{Anti-clustering in the national SARS-CoV-2 daily infection counts}",
      journal = {arXiv e-prints},
     keywords = {Quantitative Biology - Populations and Evolution, Physics - Physics and Society, Statistics - Methodology},
         year = 2020,
        month = jul,
          eid = {arXiv:2007.11779},
        pages = {arXiv:2007.11779},
archivePrefix = {arXiv},
       eprint = {2007.11779},
 primaryClass = {q-bio.PE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200711779R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{aissi20,
     author = {Dylan A\"issi},
      title = "{Review for Towards Long-term and Archivable Reproducibility}",
       year = {2020},
    journal = {Authorea},
     volume = {n/a},
      pages = {n/a},
        doi = {10.22541/au.159724632.29528907},

}





@ARTICLE{mesnard20,
     author = {Olivier Mesnard and Lorena A. Barba},
      title = {Reproducible Workflow on a Public Cloud for Computational Fluid Dynamics},
       year = {2020},
    journal = {Computing in Science \& Engineering},
     volume = {22},
      pages = {102-116},
        doi = {10.1109/MCSE.2019.2941702},
}





@ARTICLE{dicosmo20,
       author = {{Di Cosmo}, Roberto and {Gruenpeter}, Morane and {Zacchiroli}, Stefano},
        title = "{Referencing Source Code Artifacts: a Separate Concern in Software Citation}",
      journal = {Computing in Science \& Engineering},
         year = 2020,
       volume = 22,
          eid = {arXiv:2001.08647},
        pages = {33},
archivePrefix = {arXiv},
       eprint = {2001.08647},
 primaryClass = {cs.DL},
          doi = {10.1109/MCSE.2019.2963148},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200108647D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{hinsen20,
     author = {Konrad Hinsen},
      title = {The Magic of Content-Addressable Storage},
       year = {2020},
    journal = {Computing in Science \& Engineering},
     volume = {22},
     number = {03},
      pages = {113-119},
        doi = {10.1109/MCSE.2019.2949441},
}




@ARTICLE{menke20,
     author = {Joe Menke and Martijn Roelandse and Burak Ozyurt and Maryann Martone and Anita Bandrowski},
      title = {Rigor and Transparency Index, a new metric of quality for assessing biological and medical science methods},
       year = {2020},
    journal = {iScience},
     volume = {23},
      issue = {11},
      pages = {101698},
        doi = {10.1016/j.isci.2020.101698},
}





@ARTICLE{nust20,
     author = {Daniel N\"ust and Vanessa Sochat and Ben Marwick and Stephen J. Eglen and Tim Head and Tony Hirst and Benjamin D. Evans},
      title = "{Ten simple rules for writing Dockerfiles for reproducible data science}",
       year = {2020},
    journal = {PLOS Computational Biology},
     volume = {16},
      pages = {e1008316},
        doi = {10.1371/journal.pcbi.1008316},
}





@ARTICLE{konkol20,
       author = {{Konkol}, Markus and {N{\"u}st}, Daniel and {Goulier}, Laura},
        title = "{Publishing computational research -- A review of infrastructures for reproducible and transparent scholarly communication}",
      journal = {arXiv},
         year = 2020,
        month = jan,
        pages = {2001.00484},
archivePrefix = {arXiv},
       eprint = {2001.00484},
 primaryClass = {cs.DL},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200100484K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{infante20,
       author = {{Infante-Sainz}, Ra{\'u}l and {Trujillo}, Ignacio and
         {Rom{\'a}n}, Javier},
        title = "{The Sloan Digital Sky Survey extended point spread functions}",
      journal = {Monthly Notices of the Royal Astronomical Society},
     keywords = {instrumentation: detectors, methods: data analysis, techniques: image processing, techniques: photometric, galaxies: haloes, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2020",
        month = "Feb",
       volume = {491},
       number = {4},
        pages = {5317-5329},
          doi = {10.1093/mnras/stz3111},
archivePrefix = {arXiv},
       eprint = {1911.01430},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5317I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{gibney20,
     author = {Elizabeth Gibney},
      title = "{This AI researcher is trying to ward off a reproducibility crisis}",
       year = {2020},
    journal = {Nature},
     volume = {577},
      pages = {14},
        doi = {10.1038/d41586-019-03895-5},
}





@ARTICLE{lofstead19,
     author = {Jay Lofstead and Joshua Baker and Andrew Younge},
      title = {Data Pallets: Containerizing Storage for Reproducibility and Traceability},
       year = {2019},
    journal = {High Performance Computing. ISC High Performance 2019},
     volume = {11887},
      pages = {1},
        doi = {10.1007/978-3-030-34356-9\_4},
}





@ARTICLE{clement19,
     author = {Cl\'ement-Fontaine, M\'elanie and Di Cosmo, Roberto and Guerry, Bastien and MOREAU, Patrick and Pellegrini, Fran\c cois},
      title = {Encouraging a wider usage of software derived from research},
       year = {2019},
    journal = {Archives ouvertes HAL},
     volume = {},
      pages = {\href{https://hal.archives-ouvertes.fr/hal-02545142}{hal-02545142}},
}





@ARTICLE{pimentel19,
     author = {{Jo\~ao Felipe} Pimentel and Leonardo Murta and Vanessa Braganholo and Juliana Freire},
      title = {A large-scale study about quality and reproducibility of jupyter notebooks},
       year = {2019},
    journal = {Proceedings of the 16th International Conference on Mining Software Repositories},
     volume = {1},
      pages = {507-517},
        doi = {10.1109/MSR.2019.00077},
}





@ARTICLE{miksa19a,
     author = {Tomasz Miksa and Paul Walk and Peter Neish},
      title = "{RDA DMP Common Standard for Machine-actionable Data Management Plans}",
       year = {2019},
    journal = {RDA},
      pages = {doi:10.15497/rda00039},
        doi = {10.15497/rda00039},
}





@ARTICLE{miksa19b,
     author = {Tomasz Miksa and Stephanie Simms and Daniel Mietchen and Sarah Jones},
      title = {Ten principles for machine-actionable data management plans},
       year = {2019},
    journal = {PLoS Computational Biology},
     volume = {15},
      pages = {e1006750},
        doi = {10.1371/journal.pcbi.1006750},
}





@ARTICLE{dicosmo19,
     author = {M\'elanie Cl\'ement-Fontaine and Roberto Di Cosmo and Bastien Guerry and Patrick Moreau and Francois Pellegrini},
      title = {Encouraging a wider usage of software derived from research},
       year = {2019},
    journal = {Ouvrir la science},
     volume = {},
      pages = {\href{https://hal.archives-ouvertes.fr/hal-02545142}{hal-02545142}},
        doi = {},
}





@ARTICLE{perignon19,
     author = {Christophe P\'erignon and Kamel Gadouche and Christophe Hurlin and Roxane Silberman and Eric Debonnel},
      title = {Certify reproducibility with confidential data},
       year = {2019},
    journal = {Science},
     volume = {365},
      pages = {127},
        doi = {10.1126/science.aaw2825},
}





@ARTICLE{munafo19,
     author = {Marcus Munaf\'o},
      title = {Raising research quality will require collective action},
       year = {2019},
    journal = {Nature},
     volume = {576},
      pages = {183},
        doi = {10.1038/d41586-019-03750-7},
}





@ARTICLE{jones19,
       author = {{Jones}, M.~G. and {Verdes-Montenegro}, L. and {Damas-Segovia}, A. and
         {Borthakur}, S. and {Yun}, M. and {del Olmo}, A. and {Perea}, J. and
         {Rom{\'a}n}, J. and {Luna}, S. and {Lopez Gutierrez}, D. and
         {Williams}, B. and {Vogt}, F.~P.~A. and {Garrido}, J. and
         {Sanchez}, S. and {Cannon}, J. and {Ram{\'\i}rez-Moreta}, P.},
        title = "{Evolution of compact groups from intermediate to final stages. A case study of the H I content of HCG 16}",
      journal = {Astronomy \& Astrophysics},
       eprint = {1910.03420},
     keywords = {galaxies: groups: individual: HCG 16, galaxies: interactions, galaxies: evolution, galaxies: ISM, radio lines: galaxies},
         year = "2019",
        month = "Dec",
       volume = {632},
          eid = {A78},
        pages = {A78},
          doi = {10.1051/0004-6361/201936349},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A..78J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{banek19,
       author = {{Banek}, Christine and {Thornton}, Adam and {Economou}, Frossie and
         {Fausti}, Angelo and {Krughoff}, K. Simon and {Sick}, Jonathan},
        title = "{Why is the LSST Science Platform built on Kubernetes?}",
      journal = {Proceedings of ADASS XXIX},
       volume = {arXiv},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2019",
        month = "Nov",
          eid = {arXiv:1911.06404},
        pages = {1911.06404},
archivePrefix = {arXiv},
       eprint = {1911.06404},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191106404B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{fineberg19,
     author = {Harvey V. Fineberg and David B. Allison and Lorena A. Barba and Dianne Chong and David L. Donoho and Juliana Freire and Gerald Gabrielse and Constantine Gatsonis and Edward Hall and Thomas H. Jordan and Dietram A. Scheufele and Victoria Stodden and Simine Vazire, Timothy D. Wilson and Wendy Wood and Jennifer Heimberg and Thomas Arrison and Michael Cohen and Michele Schwalbe and Adrienne Stith Butler and Barbara A. Wanchisen and Tina Winters and Rebecca Morgan and Thelma Cox and Lesley Webb and Garret Tyson and Erin Hammers Forstag},
      title = {Reproducibility and Replicability in Science},
    journal = {The National Academies Press},
       year = 2019,
      pages = {1-256},
        doi = {10.17226/25303},
}





@ARTICLE{akhlaghi19,
       author = {{Akhlaghi}, Mohammad},
        title = "{Carving out the low surface brightness universe with NoiseChisel}",
      journal = {IAU Symposium 355},
       volume = {\,},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Computer Science - Computer Vision and Pattern Recognition},
         year = "2019",
        month = "Sep",
          eid = {arXiv:1909.11230},
        pages = {},
archivePrefix = {arXiv},
       eprint = {1909.11230},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190911230A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{cribbs19,
     author = {Cribbs, AP and Luna-Valero, S and George, C and Sudbery, IM and Berlanga-Taylor, AJ and Sansom, SN and Smith, T and Ilott, NE and Johnson, J and Scaber, J and Brown, K and Sims, D and Heger, A},
      title = {CGAT-core: a python framework for building scalable, reproducible computational biology workflows [version 2; peer review: 1 approved, 1 approved with reservations]},
    journal = {F1000Research},
       year = 2019,
     volume = 8,
      pages = {377},
        doi = {10.12688/f1000research.18674.2},
}





@ARTICLE{kurtzer17,
     author = {Gregory M. Kurtzer and Vanessa Sochat and Michael W. Bauer},
      title = {Singularity: Scientific containers for mobility of compute},
    journal = {PLoS ONE},
       year = {2017},
     volume = {12},
      pages = {e0177459},
        doi = {10.1371/journal.pone.0177459},
}





@ARTICLE{meng17,
     author = {Haiyan Meng and Douglas Thain},
      title = {Facilitating the Reproducibility of Scientific Workflows with Execution Environment Specifications},
    journal = {Procedia Computer Science},
       year = {2017},
     volume = {108},
      pages = {705},
        doi = {10.1016/j.procs.2017.05.116},
}





@ARTICLE{tommaso17,
     author = {Paolo Di Tommaso and Maria Chatzou and Evan W Floden and Pablo Prieto Barja and Emilio Palumbo and Cedric Notredame},
      title = {Nextflow enables reproducible computational workflows},
    journal = {Nature Biotechnology},
       year = 2017,
     volume = 35,
      pages = 316,
        doi = {10.1038/nbt.3820},
}





@ARTICLE{brinckman17,
     author = {Adam Brinckman and Kyle Chard and Niall Gaffney and Mihael Hategan and Matthew B. Jones and Kacper Kowalik and Sivakumar Kulasekaran and Bertram Ludäscher and Bryce D. Mecum and Jarek Nabrzyski and Victoria Stodden and Ian J. Taylor and Matthew J. Turk and Kandace Turner},
      title = {Computing environments for reproducibility: Capturing the ``Whole Tale''},
    journal = {Future Generation Computer Systems},
       year = 2017,
     volume = 94,
      pages = 854,
        doi = {10.1016/j.future.2017.12.029},
}





@ARTICLE{uhse19,
       author = {Uhse, Simon and Pflug, Florian G. and {von Haeseler}, Arndt and Djamei, Armin},
        title = {Insertion Pool Sequencing for Insertional Mutant Analysis in Complex Host‐Microbe Interactions},
      journal = {Current Protocols in Plant Biology},
       volume = {4},
         year = "2019",
        month = "July",
        pages = {e20097},
          doi = {10.1002/cppb.20097},
}





@ARTICLE{alliez19,
       author = {{Alliez}, Pierre and {Di Cosmo}, Roberto and {Guedj}, Benjamin and
         {Girault}, Alain and {Hacid}, Mohand-Said and {Legrand}, Arnaud and
         {Rougier}, Nicolas P.},
        title = "{Attributing and Referencing (Research) Software: Best Practices and Outlook from Inria}",
      journal = {Computing in Science \& Engineering},
       volume = {22},
     keywords = {Computer Science - Digital Libraries, Computer Science - Software Engineering},
         year = "2019",
        month = "May",
        pages = {39-52},
archivePrefix = {arXiv},
       eprint = {1905.11123},
 primaryClass = {cs.DL},
          doi = {10.1109/MCSE.2019.2949413},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190511123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kneller19,
       author = {Kneller,Gerald R. and Hinsen,Konrad},
        title = {Memory effects in a random walk description of protein structure ensembles},
      journal = {The Journal of Chemical Physics},
       volume = {150},
         year = {2019},
        pages = {064911},
          doi = {10.1063/1.5054887},
}





@ARTICLE{oliveira18,
       author = {Lu\'is Oliveira and David Wilkinson and Daniel Moss\'e and Bruce Robert Childers},
        title = {Supporting Long-term Reproducible Software Execution},
      journal = {Proceedings of the First International Workshop on Practical Reproducible Evaluation of Computer Systems (P-RECS'18)},
       volume = {1},
         year = {2018},
        pages = {6},
          doi = {10.1145/3214239.3214245},
}





@ARTICLE{rule19,
       author = {{Rule}, Adam and {Birmingham}, Amanda and {Zuniga}, Cristal and
                 {Altintas}, Ilkay and {Huang}, Shih-Cheng and {Knight}, Rob and
                 {Moshiri}, Niema and {Nguyen}, Mai H. and {Brin Rosenthal},
                 Sara and {P{\'e}rez}, Fernando and {Rose}, Peter W.},
        title = {Ten Simple Rules for Reproducible Research in Jupyter Notebooks},
      journal = {PLOS Computational Biology},
       volume = {15},
         year = 2019,
        month = jul,
        pages = {e1007007},
archivePrefix = {arXiv},
       eprint = {1810.08055},
          doi = {10.1371/journal.pcbi.1007007},
}





@article{tange18,
       author = {Tange, Ole},
        title = {GNU Parallel 2018},
      Journal = {Zenodo},
       volume = {1146014},
        pages = {\href{https://doi.org/10.5281/zenodo.1146014}{DOI:10.5281/zenodo.1146014}},
         year = 2018,
         ISBN = {9781387509881},
          doi = {10.5281/zenodo.1146014},
          url = {https://doi.org/10.5281/zenodo.1146014}
}





@ARTICLE{rule18,
       author = {Adam Rule and Aur\'elien Tabard and {James D.} Hollan},
        title = {Exploration and Explanation in Computational Notebooks},
      journal = {Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
       volume = {1},
         year = {2018},
        pages = {30},
          doi = {10.1145/3173574.3173606},
}





@ARTICLE{plesser18,
       author = {Hans E. Plesser},
        title = {Reproducibility vs. Replicability: A Brief History of a Confused Terminology},
      journal = {Frontiers in Neuroinformatics},
       volume = {11},
         year = {2018},
        pages = {76},
          doi = {10.3389/fninf.2017.00076},
}





@ARTICLE{zhang18,
       author = {{Zhang}, Zhi-Yu and {Romano}, D. and {Ivison}, R.~J. and
         {Papadopoulos}, Padelis P. and {Matteucci}, F.},
        title = "{Stellar populations dominated by massive stars in dusty starburst galaxies across cosmic time}",
      journal = {Nature},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Jun",
       volume = {558},
       number = {7709},
        pages = {260},
          doi = {10.1038/s41586-018-0196-x},
archivePrefix = {arXiv},
       eprint = {1806.01280},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018Natur.558..260Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{smart18,
       author = {{Smart}, A.G.},
        title = {The war over supercooled water},
      journal = {Physics Today},
       volume = {Aug},
         year = "2018",
        pages = {DOI:10.1063/PT.6.1.20180822a},
          doi = {10.1063/PT.6.1.20180822a},
}





@ARTICLE{kaiser18,
       author = {{Kaiser}, J.},
        title = {Plan to replicate 50 high-impact cancer papers shrinks to just 18},
      journal = {Science},
       volume = {Jul},
         year = "2018",
        pages = {31},
          doi = {10.1126/science.aau9619},
}





@ARTICLE{abramatic18,
       author = {Jean-Francois Abramatic and Roberto {Di Cosmo} and Stefano Zacchiroli},
        title = {Identifiers for Digital Objects: The case of software source code preservation},
      journal = {Communications of the ACM},
         year = 2018,
       volume = 61,
        issue = 10,
        pages = {29},
          doi = {10.1145/3183558},
}





@ARTICLE{dicosmo18,
       author = {{Di Cosmo}, Roberto and {Gruenpeter}, Morane and {Zacchiroli}, Stefano},
        title = {Identifiers for Digital Objects: The case of software source code preservation},
      journal = {Proceedings of iPRES 2018},
         year = "2018",
        pages = {204.4},
          doi = {10.17605/osf.io/kde56},
}





@ARTICLE{gruning18,
       author = {Gr\"uning, Bj\"orn and Chilton, John and K\"oster, Johannes and Dale, Ryan and Soranzo, Nicola and {van den Beek}, Marius and Goecks, Jeremy and Backofen, Rolf and Nekrutenko, Anton and Taylor, James},
        title = {Practical Computational Reproducibility in the Life Sciences},
      journal = {Cell Systems},
       volume = 6,
         year = "2018",
        pages = {631. bioRxiv:\href{https://www.biorxiv.org/content/10.1101/200683v2}{200683}},
          doi = {10.1016/j.cels.2018.03.014},
}





@ARTICLE{allen18,
       author = {{Allen}, Alice and {Teuben}, Peter J. and {Ryan}, P. Wesley},
        title = "{Schroedinger's Code: A Preliminary Study on Research Source Code Availability and Link Persistence in Astrophysics}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {methods: numerical, Astrophysics - Instrumentation and Methods for Astrophysics, Computer Science - Digital Libraries},
         year = "2018",
        month = "May",
       volume = {236},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/1538-4365/aab764},
archivePrefix = {arXiv},
       eprint = {1801.02094},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..236...10A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{burrell18,
       author = {{Burrell}, A.G. and {Halford}, A. and {Klenzing}, J. and {Stoneback}, R.A. and {Morley}, S.K. and {Annex}, A.M. and {Laundal}, K.M. and {Kellerman}, A.C. and {Stansby}, D. and {Ma}, J.},
        title = {Snakes on a Spaceship—An Overview of Python in Heliophysics},
      journal = {Journal of Geophysical Research: Space Physics},
       volume = {123},
         year = "2018",
        pages = {384},
          doi = {10.1029/2018JA025877},
}





@article{stodden18,
        author = {{Stodden}, V. and {Seiler}, J. and {Ma}, Z.},
        title = {An empirical analysis of journal policy effectiveness for computational reproducibility},
        volume = {115},
        number = {11},
        pages = {2584},
        year = {2018},
        doi = {10.1073/pnas.1708290115},
        issn = {0027-8424},
        URL = {https://www.pnas.org/content/115/11/2584},
        journal = {Proceedings of the National Academy of Sciences}
}





@article {fanelli18,
        author = {{Fanelli}, D.},
        title = {Opinion: Is science really facing a reproducibility crisis, and do we need it to?},
        volume = {115},
        number = {11},
        pages = {2628},
        year = {2018},
        doi = {10.1073/pnas.1708272114},
        publisher = {National Academy of Sciences},
        issn = {0027-8424},
        URL = {https://www.pnas.org/content/115/11/2628},
        journal = {Proceedings of the National Academy of Sciences}
}






@ARTICLE{lewis18,
       author = {{Lewis}, L.M. and {Edwards}, M.C. and {Meyers}, Z.R. and {Conover Talbot}, C. and {Hao}, H. and {Blum}, D. },
        title = "{Replication Study: Transcriptional amplification in tumor cells with elevated c-Myc}",
      journal = {eLife},
       volume = {7},
         year = "2018",
        month = "January",
        pages = {e30274},
          doi = {10.7554/eLife.30274},
}





@ARTICLE{akhlaghi18b,
       author = {{Akhlaghi}, Mohammad and {Bacon}, Roland and {Inami}, Hanae},
        title = "{MUSE HUDF survey I \& II, Sections 7.3 \& 3.4: photometry for objects with no prior broad-band segmentation map}",
      journal = {Zenodo},
        pages = {DOI:10.5281/zenodo.1164774},
         year = "2018",
        month = "February",
          doi = {10.5281/zenodo.1164774},
}





@ARTICLE{akhlaghi18a,
       author = {{Akhlaghi}, Mohammad and {Bacon}, Roland},
        title = "{MUSE HUDF survey I, Section 4: data and reproduction pipeline for photometry and astrometry}",
      journal = {Zenodo},
        pages = {DOI:10.5281/zenodo.1163746},
         year = "2018",
        month = "January",
          doi = {10.5281/zenodo.1163746},
}





@ARTICLE{leek17,
     author = {Jeffrey T. Leek and Leah R. Jager},
      title = {Is Most Published Research Really False?},
    journal = {Annual Review of Statistics and Its Application},
     volume = {4},
       year = {2017},
      pages = {109},
        doi = {10.1146/annurev-statistics-060116-054104},
}





@ARTICLE{reich17,
     author = {Michael Reich and Thorin Tabor and Ted Liefeld and Helga Thorvaldsdóttir and Barbara Hill and Pablo Tamayo and Jill P. Mesirov},
      title = {The GenePattern Notebook Environment},
    journal = {Cell Systems},
       year = {2017},
     volume = {5},
      pages = {149},
        doi = {10.1016/j.cels.2017.07.003},
}





@ARTICLE{becker17,
       author = {Gabriel Becker and Cory Barr and Robert Gentleman and Michael Lawrence},
        title = {Enhancing Reproducibility and Collaboration via Management of R Package Cohorts},
      journal = {Journal of Statistical Software, Articles},
       volume = {82},
        pages = 1,
         year = "2017",
archivePrefix = {arXiv},
       eprint = {1501.02284},
          doi = {10.18637/jss.v082.i01},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv150102284B},
}





@ARTICLE{jenness17,
       author = {{Jenness}, Tim},
        title = "{Modern Python at the Large Synoptic Survey Telescope}",
      journal = {ADASS 27},
         year = "2017",
        month = "Dec",
          eid = {arXiv:1712.00461},
        pages = {arXiv:1712.00461},
archivePrefix = {arXiv},
       eprint = {1712.00461},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv171200461J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{bezanson17,
    title={Julia: A fresh approach to numerical computing},
    author={Bezanson, Jeff and Edelman, Alan and Karpinski, Stefan and Shah, Viral B},
    journal={SIAM {R}eview},
    volume={59},
    number={1},
    pages={65},
    year={2017},
    archivePrefix={arXiv},
    eprint={1411.1607},
    publisher={SIAM},
    doi={10.1137/141000671},
    adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1411.1607B},
}





@ARTICLE{melson17,
       author = {{Melsen}, L.A. and {Torfs}, P.J.J.F and {Uijlenhoet}, R. and {Teuling}, A.J.},
        title = {Comment on “Most computational hydrology is not reproducible, so is it really science?” by Christopher Hutton et al.},
      journal = {Water Resources Research},
       volume = 53,
        pages = {2568},
         year = {2017},
          doi = {10.1002/2016WR020208},
}





@ARTICLE{munafo17,
       author = {{Munaf\'o}, M.R. and {Nosek}, B.A. and {Bishop}, D.V.M. and {Button}, K.S. and {Chambers}, C.D. and {Percie du Sert}, N. and {Simonsohn}, U. and {Wagenmakers}, E.J. and {Ware}, J.J. {Ioannidis}, J.P.A.},
        title = {A manifesto for reproducible science},
      journal = {Nature Human Behaviour},
       volume = 1,
        pages = {21},
         year = {2017},
          doi = {10.1038/s41562-016-0021},
}





@ARTICLE{jimenez17,
  title={The popper convention: Making reproducible systems evaluation practical},
       author = {{Jimenez}, I. and {Sevilla}, M. and {Watkins}, N. and {Maltzahn}, C. and {Lofstead}, J. and {Mohror}, K. and {Arpaci-Dusseau}, A. and {Arpaci-Dusseau}, R.},
      journal = {IEEE IPDPSW},
        pages = {1561},
         year = {2017},
          doi = {10.1109/IPDPSW.2017.157},
}





@ARTICLE{bacon17,
       author = {{Bacon}, Roland and {Conseil}, Simon and {Mary}, David and
         {Brinchmann}, Jarle and {Shepherd}, Martin and {Akhlaghi}, Mohammad and
         {Weilbacher}, Peter M. and {Piqueras}, Laure and {Wisotzki}, Lutz and
         {Lagattuta}, David and {Epinat}, Benoit and {Guerou}, Adrien and
         {Inami}, Hanae and {Cantalupo}, Sebastiano and
         {Courbot}, Jean Baptiste and {Contini}, Thierry and {Richard}, Johan and
         {Maseda}, Michael and {Bouwens}, Rychard and {Bouch{\'e}}, Nicolas and
         {Kollatschny}, Wolfram and {Schaye}, Joop and {Marino}, Raffaella Anna and
         {Pello}, Roser and {Herenz}, Christian and {Guiderdoni}, Bruno and
         {Carollo}, Marcella},
        title = "{The MUSE Hubble Ultra Deep Field Survey. I. Survey description, data reduction, and source detection}",
      journal = {Astronomy \& Astrophysics},
     keywords = {galaxies: distances and redshifts, galaxies: high-redshift, cosmology: observations, methods: data analysis, techniques: imaging spectroscopy, galaxies: formation, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Nov",
       volume = {608},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201730833},
archivePrefix = {arXiv},
       eprint = {1710.03002},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A\&A...608A...1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{austin17,
       author = {{Claire C.} Austin and Theodora Bloom and Sünje Dallmeier-Tiessen and {Varsha K.} Khodiyar and Fiona Murphy and Amy Nurnberger and Lisa Raymond and Martina Stockhause and Jonathan Tedds and Mary Vardigan and Angus Whyte},
        title = {Key components of data publishing: using current best practices to develop a reference model for data publishing},
      journal = {International Journal on Digital Libraries},
       volume = {18},
         year = {2017},
        pages = {77-92},
          doi = {10.1007/s00799-016-0178-2},
}





@ARTICLE{chirigati16,
       author = {Chirigati, Fernando and Rampin, R{\'e}mi and Shasha, Dennis and Freire, Juliana},
        title = {ReproZip: Computational Reproducibility With Ease},
      journal = {Proceedings of the 2016 International Conference on Management of Data (SIGMOD 16)},
       volume = {2},
         year = {2016},
        pages = {2085},
          doi = {10.1145/2882903.2899401},
}





@ARTICLE{smith16,
       author = {Arfon M. Smith and Daniel S. Katz and Kyle E. Niemeyer},
        title = {Software citation principles},
      journal = {PeerJ Computer Science},
       volume = {2},
         year = {2016},
        pages = {e86},
          doi = {10.7717/peerj-cs.86},
}





@ARTICLE{ziemann16,
       author = {Mark Ziemann and Yotam Eren and Assam El-Osta},
        title = {Gene name errors are widespread in the scientific literature},
      journal = {Genome Biology},
       volume = {17},
         year = {2016},
        pages = {177},
          doi = {10.1186/s13059-016-1044-7},
}





@ARTICLE{hinsen16,
       author = {Konrad Hinsen},
        title = {Scientific notations for the digital era},
      journal = {The Self Journal of Science},
         year = {2016},
        pages = {1: arXiv:\href{https://arxiv.org/abs/1605.02960}{1605.02960}},
}





@ARTICLE{kluyver16,
       author = {Thomas Kluyver and Benjamin Ragan-Kelley and Fernando Pérez and Brian Granger and Matthias Bussonnier and Jonathan Frederic and Kyle Kelley and Jessica Hamrick and Jason Grout and Sylvain Corlay and Paul Ivanov and Damián Avila and Safia Abdalla and Carol Willing},
        title = "{Jupyter Notebooks – a publishing format for reproducible computational workflows}",
      journal = {Positioning and Power in Academic Publishing: Players, Agents and Agendas},
         year = {2016},
        pages = {87},
          doi = {10.3233/978-1-61499-649-1-87},
}





@ARTICLE{baker16,
       author = {{Baker}, M.},
        title = "{Is there a reproducibility crisis?}",
      journal = {Nature},
       volume = {533},
         year = "2016",
        month = "May",
        pages = {452},
          doi = {10.1038/533452a},
}





@ARTICLE{wilkinson16,
     author = { {Wilkinson}, M.D and {Dumontier}, M. and {Aalbersberg}, I.J. and {Appleton}, G. and {Axton}, M. and {Baak}, A. and {Blomberg}, N. and {Boiten}, J. and {da Silva Santos}, L.B and {Bourne}, P.E. and {Bouwman}, J. and {Brookes}, A.J. and {Clark}, T. and {Crosas}, M. and {Dillo}, I. and {Dumon}, O. and {Edmunds}, S. and {Evelo}, C. and {Finkers}, R. and {Gonzalez-Beltran}, A. and {Gray}, A.J.G. and {Groth}, P. and {Goble}, C. and {Grethe}, Jeffrey S. and {Heringa}, J. and {’t Hoen}, P.A.C and {Hooft}, R. and {Kuhn}, T. and {Kok}, R. and {Kok}, J. and {Lusher}, S. and {Martone}, M. and {Mons}, A. and {Packer}, A. and {Persson}, B. and {Rocca-Serra}, P. and {Roos}, M. and {van Schaik}, R. and {Sansone}, S. and {Schultes}, E. and {Sengstag}, T. and {Slater}, T. and {Strawn}, G. and {Swertz}, M. and {Thompson}, M. and {van der Lei}, J. and {van Mulligen}, E. and {Velterop}, J. and {Waagmeester}, A. and {Wittenburg}, P. and {Wolstencroft}, K. and {Zhao}, J. and {Mons}, B.},
      title = "{The FAIR Guiding Principles for scientific data management and stewardship}",
    journal = {Scientific Data},
       year = 2016,
      month = mar,
     volume = 3,
      pages = {160018},
        doi = {10.1038/sdata.2016.18},
}




@ARTICLE{hutton16,
     author = {{Hutton}, C. and {Wagener}, T. and {Freer}, J. and {Han}, D. and {Duffy}, C. and {Arheimer}, B.},
      title = {Most computational hydrology is not reproducible, so is it really science?},
    journal = {Water Resources Research},
       year = {2016},
     volume = 52,
      pages = {7548},
        doi = {10.1002/2016WR019285},
}





@ARTICLE{topalidou16,
     author = {{Topalidou}, M. and {Leblois}, A. and {Boraud}, T. and {Rougier}, N.P.},
      title = {A long journey into reproducible computational neuroscience},
    journal = {Frontiers in Computational Neuroscience},
       year = {2016},
     volume = 9,
      pages = {30},
        doi = {10.3389/fncom.2015.00030},
}





@ARTICLE{gil16,
     author = {{Gil}, Yolanda and {David}, C.H. and {Demir}, I. and {Essawy}, B.T. and {Fulweiler}, R.W. and {Goodall}, J.L. and {Karlstrom}, L. and {Lee}, H. and {Mills}, H.J. and {Oh}, J. and {Pierce}, S.A. and {Pope}, A. and {Tzeng}, M.W. and {Villamizar}, S.R. and {Yu}, X},
      title = {Toward the Geoscience Paper of the Future: Best practices for documenting and sharing research from data to software to provenance},
    journal = {Earth and Space Science},
       year = 2016,
     volume = 3,
      pages = {388},
        doi = {10.1002/2015EA000136},
}





@ARTICLE{romine15,
     author = {Charles H. Romine},
      title = {Secure Hash Standard (SHS)},
    journal = {Federal Information processing standards publication},
     volume = {180},
      pages = {4},
       year = {2015},
        doi = {10.6028/NIST.FIPS.180-4},
}





@ARTICLE{horvath15,
     author = {Steve Horvath},
      title = "{Erratum to: DNA methylation age of human tissues and cell types}",
    journal = {Genome Biology},
     volume = {16},
      pages = {96},
       year = {2015},
        doi = {10.1186/s13059-015-0649-6},
}





@ARTICLE{chang15,
     author = {Andrew C. Chang and Phillip Li},
      title = {Is Economics Research Replicable? Sixty Published Papers from Thirteen Journals Say ``Usually Not''},
    journal = {Finance and Economics Discussion Series 2015-083},
       year = {2015},
      pages = {1},
        doi = {10.17016/FEDS.2015.083},
}





@ARTICLE{schaffer15,
       author = {Jonathan Schaffer},
        title = {What Not to Multiply Without Necessity},
      journal = {Australasian Journal of Philosophy},
       volume = {93},
        pages = {644},
         year = {2015},
          doi = {10.1080/00048402.2014.992447},
}





@ARTICLE{clarkso15,
     author = "Chris Clarkson and Mike Smith and Ben Marwick and Richard Fullagar and Lynley A. Wallis and Patrick Faulkner and Tiina Manne and Elspeth Hayes and Richard G. Roberts and Zenobia Jacobs and Xavier Carah and Kelsey M. Lowe and Jacqueline Matthews and S. Anna Florin",
      title = "{The archaeology, chronology and stratigraphy of Madjedbebe (Malakunanja II): A site in northern Australia with early occupation}",
    journal = {Journal of Human Evolution},
       year = 2015,
     volume = 83,
      pages = 46,
        doi = {10.1016/j.jhevol.2015.03.014},
}





@ARTICLE{meng15b,
     author = {Haiyan Meng and Douglas Thain},
      title = {Umbrella: A Portable Environment Creator for Reproducible Computing on Clusters, Clouds, and Grids},
    journal = {Proceedings of the 8th International Workshop on Virtualization Technologies in Distributed Computing (VTDC 15)},
       year = 2015,
     volume = 1,
      pages = 23,
        doi = {10.1145/2755979.2755982},
}





@ARTICLE{meng15,
     author = {Haiyan Meng and Rupa Kommineni and Quan Pham and Robert Gardner and Tanu Malik and Douglas Thain},
      title = {An invariant framework for conducting reproducible computational science},
    journal = {Journal of Computational Science},
       year = 2015,
     volume = 9,
      pages = 137,
        doi = {10.1016/j.jocs.2015.04.012},
}





@ARTICLE{gamblin15,
     author = {Gamblin, Todd and LeGendre, Matthew and Collette, Michael R. and Lee, Gregory L. and Moody, Adam and {de Supinski}, Bronis R.  and Futral, Scott},
      title = {The Spack package manager: bringing order to HPC software chaos},
    journal = {IEEE SC15},
       year = 2015,
     volume = 1,
      pages = {1},
        doi = {10.1145/2807591.2807623},
}




@ARTICLE{akhlaghi15,
     author = {{Akhlaghi}, M. and {Ichikawa}, T.},
      title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
    journal = {The Astrophysical Journal Supplement Series},
  archivePrefix = "arXiv",
     eprint = {1505.01664},
   primaryClass = "astro-ph.IM",
   keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric},
       year = 2015,
      month = sep,
     volume = 220,
        eid = {1},
      pages = {1-33},
        doi = {10.1088/0067-0049/220/1/1},
     adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
    adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{courtes15,
       author = {{Court{\'e}s}, Ludovic and {Wurmus}, Ricardo},
        title = {Reproducible and User-Controlled Software Environments in HPC with Guix},
      journal = {Euro-Par},
       volume = {9523},
     keywords = {Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Operating Systems, Computer Science - Software Engineering},
         year = {2015},
        month = {Jun},
          eid = {arXiv:1506.02822},
        pages = {arXiv:1506.02822},
archivePrefix = {arXiv},
       eprint = {1506.02822},
 primaryClass = {cs.DC},
          doi = {10.1007/978-3-319-27308-2\_47},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv150602822C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{hinsen15,
     author = {{Hinsen}, K.},
      title = {ActivePapers: a platform for publishing and archiving computer-aided research},
    journal = {F1000Research},
       year = 2015,
     volume = 3,
      pages = {289},
        doi = {10.12688/f1000research.5773.3},
}





@ARTICLE{belhajjame15,
     author = {{Belhajjame}, K. and {Zhao}, Z. and {Garijo}, D. and {Gamble}, M. and {Hettne}, K. and {Palma}, R. and {Mina}, E. and {Corcho}, O. and {Gómez-Pérez}, J.M. and {Bechhofer}, S. and {Klyne}, G. and {Goble}, C},
      title = "{Using a suite of ontologies for preserving workflow-centric research objects}",
    journal = {Journal of Web Semantics},
       year = 2015,
     volume = 32,
      pages = {16},
        doi = {10.1016/j.websem.2015.01.003},
}





@ARTICLE{bechhofer13,
     author = {{Bechhofer}, S. and {Buchan}, I. and {De Roure}, D. and {Missier}, P. and {Ainsworth}, J. and {Bhagat}, J. and Couch, P. and Cruickshank, D. and {Delderfield}, M and Dunlop, I. and {Gamble}, M. and {Michaelides}, D. and {Owen}, S. and {Newman}, D. and {Sufi}, S. and {Goble}, C},
      title = "{Why linked data is not enough for scientists}",
    journal = {Future Generation Computer Systems},
       year = 2013,
     volume = 29,
      pages = {599},
        doi = {10.1016/j.future.2011.08.004},
}





@ARTICLE{peng15,
     author = {{Peng}, R.D.},
      title = {The reproducibility crisis in science: A statistical counterattack},
    journal = {Significance},
       year = 2015,
      month = jun,
     volume = 12,
      pages = {30},
        doi = {10.1111/j.1740-9713.2015.00827.x},
}





@ARTICLE{dolfi14,
       author = {{Dolfi}, M. and {Gukelberger}, J. and {Hehn}, A. and
                 {Imri{\v{s}}ka}, J. and {Pakrouski}, K. and {R{\o}nnow},
                 T.~F. and {Troyer}, M. and {Zintchenko}, I. and {Chirigati},
                 F. and {Freire}, J. and {Shasha}, D.},
        title = "{A model project for reproducible papers: critical temperature for the Ising model on a square lattice}",
      journal = {arXiv},
         year = 2014,
        month = jan,
          eid = {arXiv:1401.2000},
        pages = {arXiv:1401.2000},
archivePrefix = {arXiv},
       eprint = {1401.2000},
 primaryClass = {cs.CE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1401.2000D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{katz14,
     author = {Daniel S. Katz},
      title = {Transitive Credit as a Means to Address Social and Technological Concerns Stemming from Citation and Attribution of Digital Products},
    journal = {Journal of Open Research Software},
       year = {2014},
     volume = {2},
      pages = {e20},
        doi = {10.5334/jors.be},
}





@ARTICLE{herndon14,
     author = {Thomas Herndon and Michael Ash and Robert Pollin},
      title = "{Does high public debt consistently stifle economic growth? A critique of Reinhart and Rogoff}",
    journal = {Cambridge Journal of Economics},
       year = {2014},
      month = {dec},
     volume = {38},
      pages = {257},
        doi = {10.1093/cje/bet075},
}





@ARTICLE{easterbrook14,
     author = {{Easterbook}, S.},
      title = {Open code for open science?},
    journal = {Nature Geoscience},
       year = 2014,
      month = oct,
     volume = 7,
      pages = {779},
        doi = {10.1038/ngeo2283},
}





@ARTICLE{fomel13,
     author = {Sergey Fomel and Paul Sava and Ioan Vlad and Yang Liu and Vladimir Bashkardin},
      title = {Madagascar: open-source software project for multidimensional data analysis and reproducible computational experiments},
    journal = {Journal of open research software},
       year = {2013},
     volume = {1},
      pages = {e8},
        doi = {10.5334/jors.ag},
}





@ARTICLE{sandve13,
     author = {{Sandve}, G.K. and {Nekrutenko}, A. and {Taylor}, J. and {Hovig}, E.},
      title = {Ten Simple Rules for Reproducible Computational Research},
    journal = {PLoS Computational Biology},
       year = 2013,
      month = oct,
     volume = 9,
      pages = {e1003285},
        doi = {10.1371/journal.pcbi.1003285},
}





@ARTICLE{malik13,
     author = {Tanu Malik and Quan Pham and Ian Foster},
      title = {SOLE: Towards Descriptive and Interactive Publications},
    journal = {Implementing Reproducible Research},
       year = 2013,
     volume = {Chapter 2},
      pages = {1. URL: \url{https://osf.io/ns2m3}},
}





@ARTICLE{koster12,
     author = {Johannes K\"oster and Sven Rahmann},
      title = {Snakemake—a scalable bioinformatics workflow engine},
    journal = {Bioinformatics},
     volume = {28},
      issue = {19},
       year = {2012},
      pages = {2520},
        doi = {10.1093/bioinformatics/bts480},
}





@ARTICLE{gronenschild12,
     author = {Ed H. B. M. Gronenschild and Petra Habets and Heidi I. L. Jacobs and Ron Mengelers and Nico Rozendaal and Jim van Os and Machteld Marcelis},
      title = "{The Effects of FreeSurfer Version, Workstation Type, and Macintosh Operating System Version on Anatomical Volume and Cortical Thickness Measurements}",
    journal = {PLoS ONE},
     volume = {7},
       year = {2012},
      pages = {e38234},
        doi = {10.1371/journal.pone.0038234},
}





@ARTICLE{pham12,
     author = {Quan Pham and Tanu Malik and Ian Foster and Roberto {Di Lauro} and Raffaele Montella},
      title = {SOLE: Linking Research Papers with Science Objects},
    journal = {Provenance and Annotation of Data and Processes (IPAW)},
       year = {2012},
      pages = {203},
        doi = {10.1007/978-3-642-34222-6\_16},
}





@ARTICLE{davison12,
     author = {Andrew Davison},
      title = {Automated Capture of Experiment Context for Easier Reproducibility in Computational Research},
    journal = {Computing in Science \& Engineering},
     volume = {14},
       year = {2012},
      pages = {48},
        doi = {10.1109/MCSE.2012.41},
}





@ARTICLE{zhao12,
     author = {Jun Zhao and Jose Manuel Gomez-Perez and Khalid Belhajjame and Graham Klyne and Esteban Garcia-Cuesta and Aleix Garrido and Kristina Hettne and Marco Roos and David {De Roure} and Carole Goble},
      title = {Why workflows break — Understanding and combating decay in Taverna workflows},
    journal = {IEEE 8th International Conference on E-Science},
       year = {2012},
      pages = {1},
        doi = {10.1109/eScience.2012.6404482},
}




@ARTICLE{vangorp11,
     author = {Pieter {Van Gorp} and Steffen Mazanek},
      title = {SHARE: a web portal for creating and sharing executable research},
    journal = {Procedia Computer Science},
       year = 2011,
     volume = 4,
      pages = {589},
        doi = {10.1016/j.procs.2011.04.062},
}





@ARTICLE{hinsen11,
     author = {{Hinsen}, Konrad},
      title = {A data and code model for reproducible research and executable papers},
    journal = {Procedia Computer Science},
       year = 2011,
     volume = 4,
      pages = {579},
        doi = {10.1016/j.procs.2011.04.061},
}





@ARTICLE{limare11,
     author = {Nicolas Limare and Jean-Michel Morel},
      title = {The IPOL Initiative: Publishing and Testing Algorithms on Line for
Reproducible Research in Image Processing},
    journal = {Procedia Computer Science},
       year = 2011,
     volume = 4,
      pages = {716},
        doi = {10.1016/j.procs.2011.04.075},
}





@ARTICLE{gavish11,
     author = {Matan Gavish and David L. Donoho},
      title = {A Universal Identifier for Computational Results},
    journal = {Procedia Computer Science},
       year = 2011,
     volume = 4,
      pages = {637},
        doi = {10.1016/j.procs.2011.04.067},
}




@ARTICLE{gabriel11,
     author = {Ann Gabriel and Rebecca Capone},
      title = {Executable Paper Grand Challenge Workshop},
    journal = {Procedia Computer Science},
     volume = {4},
       year = {2011},
      pages = {577},
        doi = {10.1016/j.procs.2011.04.060},
}





@ARTICLE{nowakowski11,
     author = {Piotr Nowakowski and Eryk Ciepiela and Daniel Hare\.{z}lak and Joanna Kocot and Marek Kasztelnik and Tomasz Barty\'nski and Jan Meizner and Grzegorz Dyk and Maciej Malawski},
      title = {The Collage Authoring Environment},
    journal = {Procedia Computer Science},
     volume = {4},
       year = {2011},
      pages = {608},
        doi = {j.procs.2011.04.064},
}





@ARTICLE{peng11,
     author = {{Peng}, R.D.},
      title = {Reproducible Research in Computational Science},
    journal = {Science},
       year = {2011},
      month = dec,
     volume = 334,
      pages = {1226},
        doi = {10.1126/science.1213847},
}





@ARTICLE{gil10,
     author = {Yolanda Gil and Pedro A. González-Calero and Jihie Kim and Joshua Moody and Varun Ratnakar},
      title = {A semantic framework for automatic generation of computational workflows using distributed data and component catalogues},
    journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
       year = {2010},
     volume = {23},
      pages = {389},
        doi = {10.1080/0952813X.2010.490962},
}





@ARTICLE{pence10,
       author = {{Pence}, W.~D. and {Chiappetti}, L. and {Page}, C.~G. and {Shaw}, R.~A. and
         {Stobie}, E.},
        title = "{Definition of the Flexible Image Transport System (FITS), version 3.0}",
      journal = {Astronomy and Astrophysics},
     keywords = {instrumentation: miscellaneous, methods: miscellaneous, techniques: miscellaneous, reference systems, standards, astronomical databases: miscellaneous},
         year = "2010",
        month = "Dec",
       volume = {524},
          eid = {A42},
        pages = {A42},
          doi = {10.1051/0004-6361/201015362},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A\&A...524A..42P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{goecks10,
     author = {Jeremy Goecks and Anton Nekrutenko and James Taylor},
      title = {Galaxy: a comprehensive approach for supporting accessible, reproducible, and transparent computational research in the life sciences},
    journal = {Genome Biology},
       year = {2010},
     volume = {11},
      pages = {R86},
        doi = {10.1186/gb-2010-11-8-r86},
}





@ARTICLE{merali10,
     author = {Zeeya Merali},
      title = {Computational science: ...Error},
    journal = {Nature},
       year = 2010,
     volume = 467,
      pages = {775},
        doi = {10.1038/467775a},
}





@ARTICLE{casadevall10,
     author = {{Casadevall}, A. and {Fang}, F.C},
      title = {Reproducible Science},
    journal = {Infection and Immunity},
       year = 2010,
     volume = 78,
      pages = {4972},
        doi = {10.1128/IAI.00908-10},
}





@ARTICLE{mesirov10,
     author = {{Mesirov}, J.P.},
      title = {Accessible Reproducible Research},
    journal = {Science},
       year = 2010,
     volume = 327,
      pages = {415},
        doi = {10.1126/science.1179653},
}





@ARTICLE{cheney09,
     author = {James Cheney and Laura Chiticariu and Wang-Chiew Tan},
      title = {Provenance in Databases: Why, How, and Where},
    journal = {Foundations and Trends in Databases},
       year = {2009},
     volume = {1},
      pages = {379},
        doi = {10.1561/1900000006},
}





@ARTICLE{ioannidis2009,
     author = {John P. A. Ioannidis and David B. Allison and Catherine A. Ball and Issa Coulibaly and Xiangqin Cui and Aedín C Culhane and Mario Falchi and Cesare Furlanello and Laurence Game and Giuseppe Jurman and Jon Mangion and Tapan Mehta and Michael Nitzberg and Grier P. Page and Enrico Petretto and Vera {van Noort}},
      title = {Repeatability of published microarray gene expression analyses},
    journal = {Nature Genetics},
       year = {2009},
     volume = {41},
      pages = {149},
        doi = {10.1038/ng.295},
}





@ARTICLE{fomel09,
     author = {Sergey Fomel and Jon F. Claerbout},
      title = {Reproducible Research},
    journal = {Computing in Science Engineering},
       year = {2009},
     volume = {11},
      pages = {5},
        doi = {10.1109/MCSE.2009.14},
}





@ARTICLE{baggerly09,
     author = {Keith A. Baggerly and Kevin R Coombes},
      title = {Deriving chemosensitivity from cell lines: Forensic bioinformatics and reproducible research in high-throughput biology},
    journal = {The Annals of Applied Statistics},
       year = {2009},
     volume = {3},
      pages = {1309},
        doi = {10.1214/09-AOAS291},
}





@ARTICLE{scheidegger08,
     author = {Carlos Scheidegger and David Koop and Emanuele Santos and Huy Vo and Steven Callahan and Juliana Freire and Cláudio Silva},
      title = {Tackling the Provenance Challenge one layer at a time},
    journal = {Concurrency Computation: Practice and Experiment},
       year = {2008},
     volume = {20},
      pages = {473},
        doi = {10.1002/cpe.1237},
}





@ARTICLE{moreau08,
     author = {Moreau, Luc and Ludäscher, Bertram and Altintas, Ilkay and Barga, Roger S. and Bowers, Shawn and Callahan, Steven and Chin JR., George and Clifford, Ben and Cohen, Shirley and Cohen-Boulakia, Sarah and Davidson, Susan and Deelman, Ewa and Digiampietri, Luciano and Foster, Ian and Freire, Juliana and Frew, James and Futrelle, Joe and Gibson, Tara and Gil, Yolanda and Goble, Carole and Golbeck, Jennifer and Groth, Paul and Holland, David A. and Jiang, Sheng and Kim, Jihie and Koop, David and Krenek, Ales and McPhillips, Timothy and Mehta, Gaurang and Miles, Simon and Metzger, Dominic and Munroe, Steve and Myers, Jim and Plale, Beth and Podhorszki, Norbert and Ratnakar, Varun and Santos, Emanuele and Scheidegger, Carlos and Schuchardt, Karen and Seltzer, Margo and Simmhan, Yogesh L. and Silva, Claudio and Slaughter, Peter and Stephan, Eric and Stevens, Robert and Turi, Daniele and Vo, Huy and Wilde, Mike and Zhao, Jun and Zhao, Yong},
      title = {The First Provenance Challenge},
    journal = {Concurrency Computation: Practice and Experiment},
       year = {2008},
     volume = {20},
      pages = {473},
        doi = {10.1002/cpe.1233},
}





@Article{matplotlib2007,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {CiSE},
  Volume    = {9},
  Number    = {3},
  Pages     = {90},
  abstract  = {Matplotlib is a 2D graphics package used for Python
  for application development, interactive scripting, and
  publication-quality image generation across user
  interfaces and operating systems.},
  publisher = {IEEE COMPUTER SOC},
  doi       = {10.1109/MCSE.2007.55},
  year      = 2007
}





@ARTICLE{witten2007,
     author = {Ben Witten and Bill Curry and Jeff Shragge},
      title = {A New Build Environment for SEP},
    journal = {Stanford Exploration Project},
       year = {2007},
     volume = {129},
      pages = {247: \url{http://sepwww.stanford.edu/data/media/public/docs/sep129/ben1.pdf}},
}





@ARTICLE{miller06,
     author = {Greg Miller},
      title = {A Scientist's Nightmare: Software Problem Leads to Five Retractions},
    journal = {Science},
       year = {2006},
     volume = {314},
      pages = {1856},
        doi = {10.1126/science.314.5807.1856},
}





@ARTICLE{reich06,
     author = {Michael Reich and Ted Liefeld and Joshua Gould and Jim Lerner and Pablo Tamayo and Jill P Mesirov},
      title = {GenePattern 2.0},
    journal = {Nature Genetics},
       year = {2006},
     volume = {38},
      pages = {500},
        doi = {10.1038/ng0506-500},
}





@ARTICLE{ludascher05,
     author = {Ludäs\-cher, Bertram and Altintas, Ilkay and Berkley, Chad and Higgins, Dan and Jaeger, Efrat and Jones, Matthew and Lee, Edward A. and Tao, Jing and Zhao, Yang},
      title = "{Scientific workflow management and the Kepler system}",
    journal = {Concurrency Computation: Practice and Experiment},
       year = {2006},
     volume = {18},
      pages = {1039},
        doi = {10.1002/cpe.994},
}





@ARTICLE{ioannidis05,
     author = {John P. A. Ioannidis},
      title = {Why Most Published Research Findings Are False},
    journal = {PLoS Medicine },
       year = {2005},
     volume = {2},
      pages = {e124},
        doi = {10.1371/journal.pmed.0020124},
}





@ARTICLE{bavoil05,
     author = {Louis Bavoil and Steven P. Callahan and Patricia J. Crossno and Juliana Freire and Carlos E. Scheidegger and Cláudio T. Silva and Huy T. Vo},
      title = "{VisTrails: Enabling Interactive Multiple-View Visualizations}",
    journal = {VIS 05. IEEE Visualization},
       year = {2005},
     volume = {},
      pages = {135},
        doi = {10.1109/VISUAL.2005.1532788},
}





@ARTICLE{dolstra04,
     author = {{Dolstra}, Eelco and {de Jonge}, Merijn and {Visser}, Eelco},
      title = {Nix: A Safe and Policy-Free System for Software Deployment},
    journal = {Large Installation System Administration Conference},
       year = {2004},
     volume = {18},
      pages = {79, PDF in \href{https://www.usenix.org/legacy/events/lisa04/tech/full\_papers/dolstra/dolstra.pdf}{LISA04 webpage}},
}





@ARTICLE{oinn04,
     author = {Oinn, Tom and Addis, Matthew and Ferris, Justin and Marvin, Darren and Senger, Martin and Greenwood, Mark and Carver, Tim and Glover, Kevin and Pocock, Matthew R. and Wipat, Anil and Li, Peter},
      title = {Taverna: a tool for the composition and enactment of bioinformatics workflows},
    journal = {Bioinformatics},
       year = {2004},
     volume = {20},
      pages = {3045},
        doi = {10.1093/bioinformatics/bth361},
}





@ARTICLE{schwab2000,
     author = {Matthias Schwab and Martin Karrenbach and Jon F. Claerbout},
      title = {Making scientific computations reproducible},
    journal = {Computing in Science \& Engineering},
       year = {2000},
     volume = {2},
      pages = {61},
        doi = {10.1109/5992.881708},
}





@ARTICLE{buckheit1995,
     author = {Jonathan B. Buckheit and David L. Donoho},
      title = "{WaveLab and Reproducible Research}",
    journal = {Wavelets and Statistics},
       year = {1995},
     volume = {1},
      pages = {55},
        doi = {10.1007/978-1-4612-2544-7\_5},
}





@ARTICLE{claerbout1992,
     author = {Jon F. Claerbout and Martin Karrenbach},
      title = {Electronic documents give reproducible research a new meaning},
    journal = {SEG Technical Program Expanded Abstracts},
       year = {1992},
     volume = {1},
      pages = {601-604},
        doi = {10.1190/1.1822162},
}





@ARTICLE{eker03,
     author = {Johan Eker and Jorn W Janneck and Edward A. Lee and Jie Liu and Xiaojun Liu and Jozsef Ludvig and Sonia Sachs and Yuhong Xiong and Stephen Neuendorffer},
      title = "{Taming heterogeneity - the Ptolemy approach}",
    journal = {Proceedings of the IEEE},
       year = {2003},
     volume = {91},
      pages = {127},
        doi = {10.1109/JPROC.2002.805829},
}





@ARTICLE{stevens03,
     author = {Robert Stevens and Kevin Glover and Chris Greenhalgh and Claire Jennings and Simon Pearce and Peter Li and Melena Radenkovic and Anil Wipat},
      title = {Performing in silico Experiments on the Grid: A Users Perspective},
    journal = {Proceedings of UK e-Science All Hands Meeting},
       year = {2003},
      pages = {43},
}





@ARTICLE{knuth84,
     author = {Donald Knuth},
      title = {Literate Programming},
    journal = {The Computer Journal},
       year = {1984},
     volume = {27},
      pages = {97},
        doi = {10.1093/comjnl/27.2.97},
}





@ARTICLE{somogyi87,
     author = {Zoltan Somogyi},
      title = {Cake: a fifth generation version of make},
    journal = {University of Melbourne},
       year = {1987},
      pages = {\href{https://pdfs.semanticscholar.org/3e97/3b5c9af7763d70cdfaabdd1b96b3b75b5483.pdf}{Corpus ID: 107669553}},
}





@ARTICLE{feldman79,
     author = {Stuart I. Feldman},
      title = {Make -- a program for maintaining computer programs},
    journal = {Journal of Software: Practice and Experience},
     volume = {9},
      pages = {255},
       year = {1979},
        doi = {10.1002/spe.4380090402},
}





@ARTICLE{mcilroy78,
     author = {M. D. McIlroy and E. N. Pinson and B. A. Tague},
      title = "{UNIX Time-Sharing System: Forward}",
    journal = {\doihref{https://archive.org/details/bstj57-6-1899/mode/2up}{Bell System Technical Journal}},
       year = {1978},
     volume = {57},
      pages = {6, ark:/13960/t0gt6xf72},
        doi = {},
}





@ARTICLE{anscombe73,
     author = {{Anscombe}, F.J.},
      title = {Graphs in Statistical Analysis},
    journal = {The American Statistician},
       year = {1973},
     volume = {27},
      pages = {17},
        doi = {10.1080/00031305.1973.10478966},
}





@ARTICLE{roberts69,
     author = {{Roberts}, K.V.},
      title = {The publication of scientific fortran programs},
    journal = {Computer Physics Communications},
       year = {1969},
     volume = {1},
      pages = {1},
        doi = {10.1016/0010-4655(69)90011-3},
}

